Deep Learning to See: Towards New Foundations of Computer Vision

The remarkable progress in computer vision over the last few years is, by and large, attributed to deep learning, fueled by the availability of huge sets of labeled data, and paired with the explosive growth of the GPU paradigm. While subscribing to this view, this book criticizes the supposed scientific progress in the field and proposes the investigation of vision within the framework of information-based laws of nature. Specifically, the present work poses fundamental questions about vision that remain far from understood, leading the reader on a journey populated by novel challenges resonating with the foundations of machine learning. The central thesis is that for a deeper understanding of visual computational processes, it is necessary to look beyond the applications of general purpose machine learning algorithms and focus instead on appropriate learning theories that take into account the spatiotemporal nature of the visual signal.

==> bk/10Q.tex <==
\section{Questions and insights}
A good way to attack important problems is to pose the right question.
John Tukey, who make outstanding contributions on the Fourier series, 
credited for the invention of the  term ``bit'',  during his research activity underlined the importance of posing
appropriate questions for an actual scientific development. In his own words:
\begin{quote}
\small
Far better an approximate answer to the right question, which is often vague, than the exact answer to the wrong question, which can always be made precise.
\end{quote}
Overall, posing appropriate questions can open a debate and solicit answers. 
However, the right questions cannot be easily posed since, while they need to 
a big pictures in mind, they also need the identification of reasonable intermediate steps. 
It is often the case that while addressing little problems, inconsistencies arise that
suggest the formulation of better questions. In this section, we formulate ten 
questions on the emergence of visual skills in nature that might contribute
to the development of a new approach to computer vision that is based
in processing of video instead of huge collections of images.

\subsection{How can we go beyond ``intensive supervision''?} 
We start with a fundamental question that reveals a commonly recognized limitation 
of nowadays studies in computer vision:
\begin{quote}{\em
{\bf Q1:} How can animals conquer visual skills without requiring ``intensive supervision''?
}\end{quote}
Everybody working in the broad area of artificial intelligence and  in the 
field of cognitive science has been stimulated by this  question. 
Yet, it has not been addressed as it definitely deserves! 
The recent remarkable achievements in  computer vision come from a 
truly different intelligent mechanism with respect to human vision 
which is based on tons of supervised examples--- 
of the order of millions. The  different environmental interactions that one can 
conceive in computers makes it possible to stress this artificial protocol of learning
that is supported by mathematical foundations  from decades and, more recently,
 by professional software tools. 
Interestingly, humans could not be exposed to such a boring interaction. Hence, 
strictly speaking, the  mechanisms behind supervised learning are truly artificial and 
offer a space for machines to conquer visual skills that humans couldn't replicate
in such a context.
Of course, there is no need to be surprised of the spectacular capabilities that machines
can achieve under such an artificial communication protocol, 
just like nobody gets surprised by the computer velocity 
in performing multiplications. 

On the other hand, because of the completely different environmental interaction, 
humans conquer the capability of recognizing objects just by a few supervisions.
If we are interested in the scientific foundations of vision, we should aspire for 
an depth explanation of this remarkable difference between humans recognition
capabilities  and nowadays computer vision technologies. 
Because of the expected saturation of performance of systems based on nowadays 
technologies, the time has already come 
to face the question. This has been advocated in a number 
of papers (see e.g.~\cite{DBLP:journals/corr/TavanaeiMM16},
\cite{Lee:2009},\cite{DBLP:conf/cvpr/RanzatoHBL07},
\cite{DBLP:conf/iccv/GoroshinBTEL15}), and the  interest in this kind of 
exploration is growing.  

It turns out that when the posed question is analyzed more carefully, one easily comes into the conclusion that the answer must be searched in the different learning communication protocols
in humans and computers. 
In a sense, we need to focus  on the role of a continuous environmental interaction during the 
``life of the agent.'' The interaction is not only carried out through symbolic communication
but, on the opposite, it seems to rely primarily on continuous-based information exchange.
The reward for successful actions is dominating the visual learning process in animals of
any specie. These actions range from drinking milk from the mother's breast to obstacle avoidance.
Hence, those actions basically result in  reinforcement learning processes that
contribute to the development of the visual skills. An eagle, like any predator, is early driven 
by the objective of capturing the prey, that strongly contributes to the development of the
visual skills. It is worth mentioning that newborns early interactions with the environment
also result in a collection of rich interactions. Just like for other primates,
the conquer of visual skills also benefits from the joint development of motion control. 
As soon as a baby begins the first experiences of object manipulation, such a task is 
paired with visual development. Successful manipulations are due to the correct visual interpretation
which, in turn, is reinforced by the concrete acts of touching and moving. Hence, this 
is just a way to ``supervise'' and reinforce visual skills as the outcome of other processes
taking place in the environment. 
% can we see without manipulating objects ? 
% can we see without binocular vision?  Binocular vision and depth perception
Interestingly, at that time, linguistic skills are nearly absent, which 
clearly indicates that, just for other animals, the learning of vision undergoes 
its own developmental phases, while the interplay with language comes later on.  

%
% genetic inheritance
%
Of course, in nature the discussion on the acquisition of vision 
cannot neglect the fundamental role of genetic inheritance, that has a fundamental
impact on the cognitive developmental steps. It is worth mentioning that 
remarkable differences have been discovered between different species of animals, 
in terms of the balance between their genome and their learning acquisition from the environment.
For example, while chicks early acquire significant visual skills~(\cite{WOOD2020104192}),
it takes months for humans, that clearly need to conquer more sophisticated 
skills at the perceptual level.

Interestingly there are intriguing 
connections with recent achievements in machine learning, where 
we have been constantly underlying the crucial role of of transfer learning 
mechanisms~(\cite{PanY09TKDE}) in many real-world problems. 
Clearly, whenever we transfer knowledge to the learning agent, this 
simplifies its own visual tasks and, as a consequence, the agent can learn
by relying on less supervised examples. However, one should bear in mind that
the current generation on neural networks that is currently used in transfer learning
is relying on the development of ``individuals'' that, as pointed out in this paper, are 
strongly limited from a ``genetic viewpoint'', since they haven't been exposed to 
visual natural interactions, which still distinguishes their features and consequent 
visual skills.

\begin{center}
\fbox{
\begin{minipage}{0.95\textwidth}\noindent \textit{
{\bf Box 1:} The bottom line is that for the posed question to be addressed one must 
dramatically change the agent environmental interactions. Interestingly, 
it is not the lack of technology for mimicking human interaction that mostly 
prevents us from going beyond ``intensive supervision'',
but the lack of a theory to support the appropriate  computational mechanisms. 
From one side, this is a truly stimulating scientific challenge. From the
other side, the development of a similar theory would likely contribute
to open new technological perspectives strongly connected with the 
local computation on thin clients --- like smartphones --- more than 
on cloud computing.
}\end{minipage}
}
\end{center}


\subsection{What is the role of time?}
As stated at the end of the previous section, a remarkable distinction 
between humans and nowadays machines is that they operate on a 
very different learning environment. 
The visual interaction that we experiment in nature leads us to 
face the following fundamental question: 
\begin{quote}{\em
{\bf Q2:} How can animals gradually conquer visual skills in their own environments?
}\end{quote} 
Apparently, we do the same by machine learning.
But, can we really state that the ``gradual'' process of human learning is somewhat 
related to the ``gradual'' weight updating of  neural networks?
 A closer look at the mechanisms that drive learning in vision tasks suggests that nowadays models
of machine learning mostly disregard the fundamental role of ``time'', which 
shouldn't be confused with the iteration steps that mark the weight update.
First, notice that  learning to see in nature takes place in a context
where the classic partition into learning and test environment is arguable.
On the other hand, this can be traced back to early ideas on statistical machine learning
and pattern recognition, which are dominated by the principles of statistics.
The collections of the training, validation, and test data lead to discover 
algorithms that are expected to find regularities in big data collections. 
This is good, yet it enables artificial processes whose underlying communication
protocol might not be adequate in many real-world problems. 
In the extreme case of batch mode learning, the protocol assumes that the agent
possesses information on its life before coming to life. 
Apparently this doesn't surprise computer vision researchers, whereas it sounds odd for the layman,
whose viewpoint shouldn't be neglected, since we might be trapped into an artificial
world created when no alternative choice was on the horizon.
The adoption of mini-batches and even the extreme solution of on-line stochastic
gradient learning are still missing a truly incorporation of time. 
Basically, they pass through the whole training data many times, a 
process which is still far apart from natural visual processes, where  
the causal structure of time dictates the gradual exposition to video sources. 
There is a notion of life-long learning  that is not  captured in nowadays computational 
schemes, since we are ignoring the role of time which imposes causality. 

Interestingly, when we start exploring the alternatives to huge collection of labelled images,
we are immediately faced with a fundamental choice, which arises when considering their 
replacement  with video collections. What about their effectiveness?
Suppose you  want to prepare a collection to be used for learning the market segment 
associated with cars (luxury vehicles, sport cars,  SUVs / off-road vehicles, ...).
It could be the case that a relatively small image database composed of a few thousands of labelled
examples is sufficient to learn the concept. 
On the other hand, in a corresponding video setting, this corresponds with a few minutes of video,
a time interval in which it is unreasonable to cover the variety of car features that can be
extracted from 10,000 images!  Basically, there will be a lot of nearly-repetitions of frames
which support scarse information with respect to the abrupt change 
from picture to picture.
%\footnote{An insightful discussion on this topic with Bastian Leibe helped
%focussing on the paradigm shift of getting around the recording of  the ``training set.''}.
This is what motivates a truly paradigm shift in the formulation of learning for vision.
In nature, it is unlikely to expect the emergence of vision from the accumulation 
of video. Hence, couldn't we do same? A new communication protocol can be defined
where the agent is simply expected to learn by processing 
the video as time goes by without its recording. While this gets rid of the need to 
accumulate and properly handle huge collections of labelled images,
the formulation of appropriate theories in this new framework is still
in its infancy.  Interestingly, this might opens great opportunities to all research centers to compete in another
battlefield.

At any stage of children development, it looks like they only acquire the visual skills that are 
required to face the current tasks.  One might believe that this is restricted to natural 
processes, but we conjecture that the temporal dimension plays 
a crucial role in the well-positioning of most challenging cognitive tasks, regardless of whether they are faced by humans or machines. 
It could be the case that the extraction of very efficient information from visual processes
that has captured the attention  for decades of computer scientists and engineers 
benefits from a sort of {\em pre-algorithmic phase}
where we primarily need to  understand basic {\em perceptual laws of vision} that hold regardless 
of the nature of the agent. This research guideline has been stimulating the conception of variational laws of learning 
that can capture the elegance and the simplicity of natural behavior~(\cite{DBLP:journals/tcs/BettiG16,DBLP:journals/corr/abs-1808-09162}).
When following this approach one promotes  the role of time by following principles that
have a very well-established tradition in physics.  Most importantly, one begins to challenge the
indisputable principle that learning can be regarded as the outcome of an optimization 
process that operates on the risk function. Clearly, there is something wrong with this 
principle in nature, since the agent doesn't possess the risk at the time of its birth!
While such a risk can be gradually constructed and the adoption of stochastic gradient 
is a definitely a great idea for capturing the underlying statistics, we are basically attacking a different problem with respect to what all species of animals are expected
to face in nature. As shown in Fig.~\ref{Scambio2-Fig}, they need to evolve over time
and, therefore, the measure $dP(x,y)$ in the classic functional risk of 
statistical machine learning is replaced with a temporal measure, with
the underlying assumption that the signal is ergodic. 
\begin{figure}[H]
	\centering
	\includegraphics[width=15cm]{figs/VA2.pdf}
\caption{\small From massive to children-like supervision. Visual agents are 
expected to learn in a truly visual environments by exploiting 
natural-language supervision. Any risk function in those environments
can be interpreted as expectations over a temporal domain.}
\label{Scambio2-Fig}
\end{figure}
In traditional machine learning we  consideri the empirical 
\begin{equation}
	E(w) = \sum_{\kappa=1}^{\ell} V(w,u_{\kappa}) + \lambda R(w)
\label{EmpiricalRisk}
\end{equation}
where $V(w,u_{\kappa})$ is a loss function\footnote{Here,  
we slightly abuse of definition ``loss function'', but the meaning is the same.} and
$R(w)$ is a regularization term properly weighed by $\lambda>0$.
A corresponding  temporal interpretation can be captured by defining the 
functional~(\cite{DBLP:journals/tnn/BettiGM20})
\begin{equation}
	E(w) = \int_{0}^{T} dt \ e^{-t/\epsilon} \bigg(\frac{\alpha \epsilon^{2}}{2} 
	\ddot{w}_{ij}^{2}(t) + 
	\frac{\beta \epsilon^{2}}{2} \dot{w}_{ij}^{2}(t)
	+ V(w_{ij}(t),u(t))\bigg)
\label{CA-Eq}
\end{equation}
where, for the sake of simplicity, we use Einstein's notation. A first interesting difference is that
this is a functional, so as $w(t)$ is clearly expected to change over $[0,T]$.
%Of course, one could have simply established a closer parallel index where $w \in \bbR^{d}$
%is the finite-dimensional vector. 
While the search for $w^{\star} = \arg \min E(w)$
can be carried out by gradient descent --- included its stochastic version --- the
basic idea behind the formulation by functional~(\ref{CA-Eq}) is that we are motivated
to discover a solution that is compatible with causality and that does not rely on the
accumulation of the training set. While the stochastic gradient algorithm can always
be a viable option,  it is still rooted in the statistical principle of cycling through 
the accumulated data. When promoting the role of time in a truly pre-algorithmic framework,
one very much would like to think of learning as a process where the weights change
over time, so as to clearly distinguish between the dynamics of the video information and the
the internal dynamics of learning. In that respect, the formulation given by Eq.~(\ref{CA-Eq}) 
imposes the direction to time, which depends on the presence of the 
factor $e^{-t/\epsilon}$. This clearly breaks time symmetry and leads to the 
irreversibility of learning. 
The analogy between
the formulations of Eq.~(\ref{EmpiricalRisk}) and Eq.~(\ref{CA-Eq}) can
promptly be seen from the presence of the loss function $V$, which can be read as
a potential in temporal framework. Likewise, the regularization term is translated into
a sort of kinetic energy, which depends on the velocity and acceleration of the
weights. The functional $E(\cdot)$ defined by Eq.~(\ref{CA-Eq}) is referred to as 
the cognitive action~(\cite{DBLP:journals/tcs/BettiG16,DBLP:journals/corr/abs-1808-09162}). 
It shares similarities and differences  with respect to the classic action
of mechanics used for handling dissipation
\begin{equation}
	S = \int_{0}^{T} dt \ e^{\theta t} \bigg( \frac{1}{2} m \dot{q}^{2} - V(q)\bigg).
\end{equation}
Clearly, there is a connection between the position of a particle, denoted by $q$, and the weights $w_{ij}$.
The kinetic energy $K= \frac{1}{2} m \dot{q}^{2}$ has in fact a counterpart in the cognitive action, where the
velocity $\dot{w}_{ij}$ 
of the weights is involved. Interestingly, also the ``acceleration of the weights'' $\ddot{w}_{ij}$ is 
involved in Eq.~(\ref{CA-Eq}). However, the discovery of laws of learning does require 
that $V(w_{ij}(t),u(t))$, which is the counterpart of the potential in mechanics, comes with the same sign as the cognitive kinetic 
energy, which is a sort of regularization term. An in-depth discussion on this issue can be 
found in~(\cite{DBLP:journals/corr/abs-1808-09162}). This action has been recently used
in~(\cite{DBLP:conf/nips/TiezziMBMG20}), where it is clearly stated that causality is gained
as $\epsilon \rightarrow 0$~(\cite{DBLP:conf/nips/TiezziMBMG20}).  Interestingly, related interpretations
of causality, to which Eq~(\ref{CA-Eq}) is inspired, has been proposed for 
mechanics~(\cite{Stefanelli2013}). It is proven that the special interpretation of the action functional given in~(\cite{Stefanelli2013})
leads to close similarities between stochastic gradient algorithms used in machine learning and 
the corresponding Euler-Lagrange equations that come from imposing the stationarity of Eq.~(\ref{CA-Eq}). 
There are  some intriguing analogies between the notion of action in mechanics and 
the cognitive action in learning theory. 
When  thinking of laws of  learning to see in the variational framework, everything comes out as a consequence of the stationarity condition of the cognitive action
\begin{equation}
	\forall t \in [0,T]: \ \ \delta E(w^{\star}(t)) = 0.
\label{VarCond}
\end{equation}
%
While there is a bridge to mechanics, the singularity that
arises by using functional~(\ref{CA-Eq}) as $\epsilon \rightarrow 0$ is basically required to gain causality so as to formulate learning
under Cauchy's conditions. Just like in machine learning, yet the initial conditions are random.
When enforcing causality by $\epsilon \rightarrow 0$, the satisfaction of Eq.~(\ref{VarCond}) somewhat
meets  stochastic gradient descent, but it does not parallel the classic related condition
\begin{equation}
	\nabla E(w^{\star}) = 0,
\label{GradEq}
\end{equation}
that is the target of the optimization. 
This is nominally achieved as the outcome of optimization when starting typically with random weights. Basically $w^{\star}$ is the final configuration of a ``temporal process'' 
connected with the internal structure of the learning agent, which is not
necessarily related to the temporal structure of the video.
On the opposite, condition~\ref{VarCond} is always supposed to hold during the agent's life.
Even though the discrete versions of Eq.~\ref{VarCond} and Eq.~\ref{GradEq} are similar, 
the underlying computational process is very different. While condition~(\ref{GradEq}) is nominally
met at the end of learning as the result of the gradient-descent, 
condition~(\ref{VarCond}) must be always satisfied.  It gives rise to Euler-Lagrange equations
that hold for any time. An in-depth understanding of the role of time does require a well-position of the
functional optimization problem for the minimization of the cognitive action. Is there any other 
way of posing the problem which does not require the degeneration of the action
defined by Eq.~(\ref{CA-Eq})?
Is $\epsilon \rightarrow 0$ the only way for incorporating causality and solve the Euler-Lagrangian 
by Cauchy's conditions? This question brings to our mind related questions on developmental
learning that we will be addressed in the remainder of the paper. What if we learn
by modifying the input? As the agent comes to life, in order to deal with the information overloading,
it makes sense to simplify rich video sources and gradually restore the actual environmental 
input as time goes by.  
For any pixel defined by $x$ at time $t$, the video $u(x,t)$
can be modified by
\begin{equation}
	\tilde{u}(x,t) = \sigma u(x,t) + \delta(x,t).
\label{InputSmooth}
\end{equation}
Consequently, a learning process can be established which satisfies
\begin{equation}
	V(w_{i,j},\tilde{u}) = 0.
\end{equation}
When following this scheme, one is forced to satisfy the constraint by the joint choice of
the connection weights and an appropriate transformation of the input $u(x,t)$ by the 
affine transformation of Eq.~(\ref{InputSmooth}).

%%%%%%%%%%%%%%%
\iffalse
Recurrent nets for action recognition - brutal supervision ... of limited importance if you consider 
the problems connected with gradient vanishing

Frame prediction on the basis of the past frames - just like in language. This is definitely better! 
It is the first clear recognition of the importance of time in vision. However, as it will be mostly
stated when discussing attention mechanisms, we are still neglecting the joint role of 
time and focus of attention. 
\fi
%%%%%%%%%%%%%%%
% time and motion invariance
%%%%%%%%%%%%%%%
The formulation of learning in the temporal dimension likely becomes more and more important when 
we begin to address a number of challenges that are also outlined in the other questions posed in the
paper. The role of time becomes crucial when considering the extraction of good features.
This is in fact an issue that, as the interest in transfer learning has been demonstrating, 
has becoming more and more relevant.  While in the literature we have been typically concerned 
with feature extraction that is independent of classic geometric transformation, it looks like we are still missing the astonishing human skill of capturing distinctive features  when looking at ironed and rumpled shirts! There is no apparent difficulty to recognize shirts by keeping the recognition coherence in case we roll up the sleeves, or we simply curl them up into a ball for the laundry basket. Of course, there are neither rigid transformations, like translations and rotation, nor scale maps that transforms an ironed shirt into the same shirt thrown into the laundry basket. 
Is there any natural invariance?

In this paper, we claim that
motion invariance is in fact the only one that we need.
%\marginnote{The paradigm-shift of motion invariance}
Translation,  scale, and rotation invariances, 
that have been the subject of many studies, are in
fact instances of invariances that can be fully gained whenever we develop the 
ability to detect features that are invariant under motion. 
If my inch moves closer and closer to my eyes then any of its representing features 
that is motion invariant will also be scale invariant. The
finger will become bigger and bigger as it approaches my face, but it is still my inch!
Clearly, translation, rotation, and complex deformation invariances  derive from
motion invariance. Humans life always experiments motion, so as the gained visual
invariances naturally arise from motion. 
Studies on different types of invariances in vision have been so rich and 
massively investigated that one can suspect  that there is something
missing in the claim that enforcing motion invariance only suffices to learn.
What if an object is gradually deformed into another one? 
One can think of cat  which is very slowly transformed
to a dog! This reminds us the metaphysical question of whether and how things 
persist over time. Philosophers regards things as concrete material objects 
as well as pure abstract objects which are associated with 
 concepts and ideas\footnote{This discussion was stimulated by
 Marcello Pelillo who pointed out intriguing links with 
 The ``Ship of Theseus Puzzle'' and ``The Puzzle of the Statue and the Clay.''}. 
Concepts can drift as video changes very slowly, which 
can deceive any intelligent agent who relies on motion invariance only, 
provided that such an agent fails detecting slow motion. 
While one can always debate on the possibility of achieving certain
thresholds for slow motion detection, when trusting motion invariance
one must be ready to accept the problem of concept drift. 
Interestingly, as will be pointed out in the reminder of the paper, 
the development of focus of attention mechanisms helps facing 
also this problem. 
 

\begin{center}
\fbox{
\begin{minipage}{0.95\textwidth}\noindent \textit{
{\bf Box 2:} The bottom line is that while we struggle for the acquisition of huge labeled databases, 
the truly incorporation of time might led to a paradigm shift in the 
process of feature extraction.
We promote the study of the agent life based on the ordinary notion of time, 
which emerges in all its facets.
The incorporation of motion invariance might be the key for overcoming the
artificial protocol of supervised learning. We claim that such an invariance 
is in fact the only one that we need.
}\end{minipage}
}
\end{center}

\subsection{Can animals see in a world of shuffled frames?}
One might figure out what human life could have been in a world of visual 
information with shuffled frames.
\begin{quote}{\em 
{\bf Q3:} Could  children really acquire visual skills in 
such an artificial world, which is the one we are presenting to machines?
Doesn't  shuffled visual frames increase the complexity of learning to see?
}\end{quote}
A related issue has been faced in~(\cite{Wood2016}) for the acquisition of 
visual skills in chicks. It is pointed out that 
``when newborn chicks  were raised with virtual objects that moved smoothly over time, 
the chicks developed accurate color recognition, shape recognition, 
and color-shape binding abilities.'' Interestingly, the authors notice that 
in contrast, ``when newborn chicks were raised with virtual objects that 
moved non-smoothly over time, the chicks' object recognition abilities were severely impaired.''
When exposed to a video
composed of independent frames  taken from a visual database, like ImageNet, that 
are presented at classic cinema frame rate
%\footnote{See SAILab experiments} 
of 24 fps,
humans seem to experiment related difficulties in non-smooth visual presentation. 
 
Hence, it turns out that our spectacular visual skills completely collapse in a task that is successfully faced
in computer vision! As a consequence, one might start formulating conjectures
on the inherent difficulty of artificial versus natural visual tasks. The remarkably 
different performance of humans and machines  has stimulated the curiosity
of many researchers in the field. 
Of course, you can start noticing that in a world of shuffled frames, a video requires order
of magnitude more information for its storing than the 
corresponding temporally coherent visual stream. 
This is a serious warning that is typically neglected in computer vision, since it suggests that
any recognition process is likely to be more difficult when shuffling
frames. One needs to extract information
by only exploiting spatial regularities in the retina, while disregarding
the spatiotemporal structure that is offered by nature. 
The removal of the thread that nature used to sew the visual frames might prevent us
from the construction of a good theory of vision. 
Basically, we need to go beyond the current scientific peaceful interlude and  
abandon the safe model of restricting computer vision to the processing of images.
%\marginnote{In modern computer vision we have been facing a
%problem that is more difficult then that offered by nature.}
%
Working with video was discouraged at the dawn of computer vision because
of the heavy computational resources that it requires, but the time has come to
reconsider significantly this implicit choice.
Not only humans and animals cannot see in a world of shuffled frames, but we also
conjecture that they could not  learn to see in such an environment.
%In a sense, the very good results that we already can experiment nowadays are 
%quite surprising, but they are mostly due to the stress of the computational power. 
%The theory proposed in this paper relies of the choice of capturing
%temporal structures in natural visual environments, which is claimed to 
%simplify dramatically the problem at hand, and to give rise to lighter computation.\\
%
%??? look for literature
%??? reference to SAILab site: Betti video
% Boccignone: Apart from CNN spaziotemporali, 
%oppure incorporano l?output di una CNN come input di una LSTM
Shuffling visual frames is the implicit assumption of most of nowadays computer vision
that, as stated in the previous section, corresponds with neglecting the role of 
time in the discovering of visual regularities. No matter what computational scheme 
we conceive, the presentation of frames where we have removed the temporal structure
exposes visual agents to a problem where a remarkable amount of information 
is delivered at any presentation of new examples. When going back to the previous
discussion on time, one clearly see its natural environmental flow that must be
somehow synchronized with the agent computational capability. 
The need for this synchronization is in fact one of the reasons for focussing attention
at specific positions in the retina, which confers the agent also the gradual 
capability of extracting information at pixel label. Moreover, as already pointed
out, we need to abandon the idea of recording a data base for  statistical assessment. 
There is nothing better than human evaluation in perceptual tasks, which could stimulate
new ways of measuring the scientific progress of the discipline (see Section~\ref{APA-sec}).

%This analysis on  ``frame shuffling'' suggests that the reasons for sticking 
%with nowadays benchmarks based on still images, along with the related computer vision
%approaches, might vanish in the next few years.
The reason for formulating a theory of learning on video instead of on images
is not only rooted in the curiosity of grasping the computational mechanisms 
that take place in nature.
A major claim in this paper is that those computational mechanisms are also fundamental
in  most of computer vision tasks.
\begin{center}
\fbox{
\begin{minipage}{0.95\textwidth}\noindent \textit{
{\bf Box 3:} It looks like that, while ignoring the crucial role of 
temporal coherence, 
the formulation of most of nowadays current computer vision tasks lead us to
tackle problems that are 
remarkably more difficult than those nature has prepared for us!
}\end{minipage}
}
\end{center}

\iffalse
%%%%%%%%%%%%%%%
{\em
It looks like that, while ignoring the crucial role of 
temporal coherence, 
the formulation of most of nowadays current computer vision tasks lead us to
tackle a problem that is 
remarkably more difficult than the one nature has prepared for us!
}
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% to be clarified
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Additional value of the smoothing: we only rely on the conditions on \sigma and \delta.
%It makes sense to think of their values on the boundaries! As we satisfy those conditions
%the conditions on w are automatically satisfied! 
%Intuition: in that case a Lagrangian with the kinetic energy limits - during minimization - 
%the problems due to instability! Is that what we are seeing in current MNIST experiments
%where we need to limit the velocity of the video? Couldn't we go faster in case we use
%4th order diff equation?

\subsection{How can humans perform  pixel semantic labeling?}
Many computer vision tasks still rely on the pattern model, that is on an
opportune pre-processing of video information represented by a vector. 
Surprisingly enough, state of the art  approaches to computer vision already
offer quite accurate scene descriptions in specific real-world contexts, without  
necessarily relying on the semantic labelling of each
pixel. A global computational scheme emerges that is typically 
made more and more effective when the environment in which the machine is supposed to 
work is quite limited, and it is known in advance. For examples, in object recognition
tasks, the number of the classes that one expect to recognize in the environment
can dramatically affect the performance. Interestingly, very high accuracy can be
achieved without necessarily being able to perform the object segmentation and, therefore, 
without needing to perform pixel semantic labeling. 
However, for an agent to conquer visual capabilities in a broad context,
it seems to be very useful to rely on appropriate primitives. 
When thinking of a video, the information that one can extract  is 
not only driven by time but also by spatial information. We humans can easily describe
a scene by locating the objects in specific positions and we can describe their eventual
movement. 
This requires a deep integration of visual and linguistic skills, that are
required to come up with compact, yet effective video descriptions. 
Based on these premises the following question naturally arises.
\begin{quote}
{\em 
{\bf Q4:} 
	How can humans exhibit such an impressive skill of properly labelling
	single pixels without having received explicit pixel-wise supervisions?
	Isn't the case that such a skill must be a sort of ``visual primitive''
	that cannot be ignored for efficiently conquering additional skills
	on object recognition and scene interpretation?
}
\end{quote}
Interestingly, in humans semantic pixel labelling is by driven by the focus of attention,
another fundamental features that, as we will see in the remainder of the paper, 
is at the core of all important computational processes of vision.
%\marginnote{Pixel-based fundamental primitives.}
While pixel-based decisions are 
inherently interwound  with a certain degree of ambiguity, they are remarkably
effective. The linguistic attributes that we can extract are related to 
the context of the pixel that is taken into account for label attachment, while
the ambiguity is mostly a linguistic more than a visual issue. 
In a sense, this primitive  is likely
in place for conquering higher abstraction levels. How can this be done?
The focus on single pixels allows us to go beyond object segmentation 
based on sliding windows.
Instead of dealing with object proposals~(\cite{DBLP:conf/eccv/ZitnickD14}),
a more primitive task is that of attaching symbols to single pixels in the retina.
The bottom line is that human-like linguistic descriptions of visual scenes 
is gained on top of pixel-based feature descriptions that, as a byproduct,
must allow us to perform semantic labeling.  The task of semantic pixel labelling
leads to process the retina by focussing attention on the given pixel, while
considering the information in its neighborhood. This clearly opens the doors
to an in-depth re-thinking of pattern recognition processes. It is not only the 
frame content, but also where we focus attention in the retina  that does matter. 

Human ability of exhibiting semantic labeling at pixel level is really challenging.
The visual developmental processes conquer this ability nearly without  
pixel-based supervisions. It seems that such a skill is mostly  the outcome of the 
acquisition of the capability to perform object segmentation. This is obtained by constructing 
the appropriate memberships of the pixels that define the segmented regions. 
When thinking of the classic human communication protocols, one early realizes that
even though it is rare to provide pixel-based supervision, 
the information that is linguistically conveyed to describe visual scenes makes implicit
reference to the focus of attention. This holds regardless of the scale of the visual entity 
being described. Hence, the emergence of the capability of performing pixel semantic
label seems to be deeply related to the emergence of focus of attention mechanisms. 
The most striking question, however, is how can humans construct such a 
spectacular segmentation without a specific pixel-based supervision! Interestingly,
we can focus on a pixel and attach meaningful labels, without having been 
instructed for that task.

\begin{center}
\fbox{
\begin{minipage}{0.95\textwidth}\noindent \textit{
{\bf Box 4:}  The primitive of pixel semantic
labelling is likely crucial for the construction of human-like visual skills. 
There should be a hidden supervisor in nature 
that, so far, has nearly been neglected.
We conjecture that it is the optical flow 
which plays the central role 
for object recognition. The decision on its recognition must be invariant under
motion, a property that does require a formulation in the temporal direction.
}\end{minipage}
}
\end{center}



% kaniska triangle foa and related examples

% WHY CAN HUMAN perform semantic labeling without supervision?

\subsection{Why receptive fields and hierarchical architectures?}
 %meziona anche approccio baysiano~\cite{Lee03hierarchicalbayesian}\\
% 
 Beginning from early studies on the visual structure of the cortex~(\cite{hubel62}), 
 neuroscientists have
gradually gained evidence on the fact that it presents a hierarchical 
structure and that neurons process the video information on the basis of inputs 
restricted to receptive fields. 
Interestingly, the recent spectacular results of convolutional neural networks 
suggests that hierarchical structures based on neural computation with 
receptive fields play a fundamental role also 
in artificial neural networks~(\cite{lecun2015deeplearning}). 
The following questions naturally arise:
%
\begin{quote}
{\bf Q5:} {\em Why are the visual mainstreams organized according to a hierarchical architecture 
with receptive fields? Is there any reason why this solution has been
developed in biology? Why is its ``replication'' in neural networks 
so successful? 
}\end{quote}
%
First of all, we can promptly realize that, even though neurons are restricted
to compute over receptive fields, deep structures rely on large virtual contexts 
for their decision.  As we increase the depth of the neural network, 
the consequent pyramidal dependence that is established by the receptive
fields increases the virtual input window used for the decision, so as higher
abstraction is progressively gained as we move towards the output. 
Hence, while one gives up to exploit all the information available at a certain
layer,  the restriction to receptive field does not prevent from 
considering large windows for the decision. The marriage of receptive fields
with deep nets turns out to be an important ingredient for a parsimonious 
and efficient implementation of  both biological and artificial networks.
In convolutional neural networks, the assumption of using receptive fields
comes with the related hypothesis of {\em weight sharing} on units that are 
supposed to extract the same feature, regardless of where the neurons are
centered in the retina. In so doing we enforce the extraction of the same 
features across the retina. This makes sense whereas, in general, it does not make sense
to extract features depending on the pixel in the retina. The same visual clues
are clearly positioned everywhere in the retina and the equality constraints on the weights
turn out to be a precise statement for implementing a sort of {\em invariance
under translation}. 

%
\iffalse
A closer look at the principle of feature extraction across the retina suggests 
that one does not necessarily need to enforce the weight sharing at 
layer level. As we move towards the output, the expressive power of the features
increases, while the principle of sharing features in different positions of the 
retina does not necessary correspond with sharing the weight of a single 
unit. The compositional power that is gained in the deep net makes it 
possibile to express the same feature, while relaxing the strong constraint of
weight sharing on the single units. The sharing involves the features more than
the structure of the single units. Hence, when associating a feature to a neuron, 
one can go beyond the request of propagating the association to its weights.
What really matters is the output of the neurons in their position in the deep structure. 
\fi
%
Clearly, this constraint has neither effect on invariance under scale nor under rotation. 
Any other form of invariance that is connected with deformable objects is clearly
missed and is supposed to be learned. The current technology of convolutional
neural networks in computer vision typically gains these invariances thanks to 
the power of supervised learning by ``brute force.'' Notice that since most
of the tasks involve object recognition in a certain environment, the associated limited 
amount of visual information allows to go beyond the principle of extracting 
visual features at pixel level. Visual features can be shared over small windows
in the retina by the process of pooling, thus limiting the dimension of the network.
Basically, the number of features to be involved has to be simply related to the
task at hand, and we can go beyond the association of the features with the
pixels. However, the conquering of human-like visual skills is not compatible with
this kind of simplifications since, as stated in the previous section, humans can
perform pixel semantic labeling. There is a corresponding trend in computer 
vision where convolutional nets are designed to keep the connection with each
pixel in the retina at any layer so as to carry out segmentation and semantic pixel
label. Interestingly, this is where we need to face a grand challenge. So far, 
very good results  have been made possible by relying on massive labelling of collections of images.
While image labeling for object classification is a  boring task, human pixel labeling 
(segmentation) is even worst! 
%There have been a number of clever techniques
%to push this research direction, which are mostly in the hand of 
%big companies like NVIDIA which offer the state of the art of this segmentation technology. 
Instead of massive supervised labelling, one could realize that motion and focus of attention
can be massively exploited to learn the visual features mostly in an unsupervised
way. A recent study in this direction is given in~(\cite{Betti2018-CN-arxiv}), 
where the authors provide evidence of the fact that
 receptive fields do 
favor the acquisition of motion invariance which, as already stated, is the 
fundamental invariance of vision. 
The study of motion invariance leads to dispute the effectiveness and the biological 
plausibility of convolutional networks. First, while weight sharing is directly gained
by translational invariance on any neuron, the vice versa clearly does not hold. 
Hence, we can think of receptive field based neurons organized in a hierarchical architecture
that carry out translation invariance without sharing their weights. 
This is strongly motivated also by the arguable biological plausibility of the 
mechanism of weight sharing~(\cite{OTT2020235}). Such a lack of plausibility 
is  more serious than the supposed lack of a truly local computational  
scheme in Backpropagation, which mostly comes from the lack of
delay in the forward model of the neurons~(\cite{DBLP:journals/corr/abs-1912-04635}).

\begin{center}
\fbox{
\begin{minipage}{0.95\textwidth}\noindent \textit{
{\bf Box 5:} Hierarchical architectures is the natural
solution for matching the notion of receptive field and 
develop abstract representations. This  also seem to 
facilitate the implementation of motion invariance, 
a property  that is at the basis of the biological structure of the visual 
cortex. The architectural incorporation of this fundamental invariance 
property, as well as the match with the need for implementing the 
focus of attention mechanisms likely need neural architectures that
are more sophisticated than current convolutional neural networks.
In particular, neurons which provide motion invariance likely benefit
from dropping the weight sharing constraint.
}\end{minipage}
}
\end{center}


\subsection{Why two  different mainstreams?}
In Section~\ref{Unbilicalsec} we have emphasized the importance of bearing in
mind the neat functional distinction between vision for action and vision for perception.
A number of studies in neuroscience lead to conclude that 
the visual cortex of humans and other primates is composed of two main information pathways
that are referred to as the  ventral stream and dorsal 
stream~(\cite{GoodaleMilner92,GOODALE1998181}).
We typically refer to  the ventral ``what'' and the dorsal ``where/how'' 
visual pathways.  The ventral stream is devoted to perceptual analysis of the visual input, such as object recognition, whereas the dorsal stream is concerned with providing spatial localization and
motion ability  in the interaction with the environment. 
The ventral stream  has strong connections to the medial temporal lobe (which stores long-term memories), the limbic system (which controls emotions), and the dorsal stream.
The dorsal stream stretches from the primary visual cortex (V1) in the occipital lobe forward into the parietal lobe. It is interconnected with the parallel ventral stream which runs downward from V1 into the temporal lobe.
\begin{quote}
{\em
{\bf Q6:}  Why are there two different mainstreams? What are the reasons for such 
a different neural evolution?
}
\end{quote}
This  neurobiological distinction arises for effectively facing visual tasks that are
very different. The exhibition of perceptual analysis and object recognition clearly requires 
computational mechanisms that are different with respect to those required for estimating the 
scale and the spatial position. Object recognition requires the ability of developing strong 
invariant properties that mostly characterize the objects themselves. By and large
scientists agree on that objects must be recognized
independently of their position in the retina, scale, and orientation. While we subscribe this point of 
view, a more careful analysis of our perceptual capabilities indicates that these desirable 
features are likely more adequate to understand the computational mechanisms 
behind the  perception  of rigid objects.
The elastic deformation and the projection into the retina gives in fact rise to remarkably more
complex patterns that can hardly be interpreted in the framework of geometrical invariances.
We reinforce the claim that {\em motion invariance is in fact the only invariance which does matter}. 
Related studies in this direction can be found~(\cite{bertasius2021spacetime}).
As the nose of a teddy bear approaches children's eyes it becomes larger and larger. Hence, 
scale invariance is just a byproduct of motion invariance. The same holds true for rotation 
invariance. Interestingly, as the children deforms the teddy bear a new visual pattern 
is created that, in any case, is the outcome of the motion of ``single object particles.'' 
The neural enforcement of motion invariance is clearly conceived 
implementing the ``what'' neurons.
Of course, neurons with built-in motion invariance are not adeguate to make spatial estimations
or detection of scale/rotation. Unlike the ``what'' neurons, in this case motion does matter
and the neural response must be affected by the movement. 

\begin{center}
\fbox{
\begin{minipage}{0.95\textwidth}\noindent \textit{
{\bf Box 6:} These analyses are  consistent with neuroanatomical evidence and suggest that 
``what'' and ``where'' neurons are important also in machines.
The anatomical difference of the two mainstreams is in fact the outcome of a truly
different functional role. While one can ignore such a difference and rely on the 
rich representational power of big deep networks, the underlined difference 
stimulates the curiosity of discovering canonical neural structures to naturally 
incorporate motion invariance, with the final purpose of discovering different features
for perception and action.  
}\end{minipage}
}
\end{center}

% ??? more details on neuroscience



\subsection{Why some animals focus attention?}
\label{Focus-section}
It is well-known that the presence of the fovea in the retina leads to focus attention on details in the scene.
Such a specialization of the visual system is widespread 
among vertebrates, it is present in some snakes and fishes, 
but among mammals is restricted to haplorhine primates.
In some nocturnal primates, like the owl monkey and in the tarsier, the fovea is morphologically distinct 
and appears to be degenerate. Owl monkey's  visual system is somewhat different from other monkeys and apes. 
As it retina develops, its dearth of cones and its surplus of rods mean
that this focal point never forms. 
Basically, a fovea is most often found in diurnal animals, thus supporting the idea that it is supposed to play an
important role for capturing details of the scene~(\cite{Ross2004}).
But why haven't many mammals developed such a rich vision system
based on foveate retinas? 
Early mammals, which emerged in the shadow of the dinosaurs, were likely forced to 
nocturnal lives so as to avoid to become their pray~(\cite{PMID:32269365}).
In his seminal monograph,  Gordon Lynn Walls~(\cite{Walls1942})
proposed that there has been a long nocturnal evolution of mammals' eyes, which
is the reason of the remarkable differences with respect to those of other vertebrates. 
The idea became known as the ``nocturnal bottleneck'' hypothesis~(\cite{Gerkema_2013}).
%Although the eyeballs of nocturnal and diurnal primates present remarkable 
%morphological differences~\cite{SCHMITZ2010936}, they share the same underlying focus of 
%attention mechanism.
Mammals' eyes tended to resemble those of nocturnal birds and lizards, but this 
does not hold for humans and closely related monkeys and apes. 
It looks they re-evolved features useful
for diurnal living after they abandoned a nocturnal lifestyle upon dinosaur extinction. 
It is worth mentioning that  haplorhine primates are not the only mammals which focus attention 
in the visual environment. Most mammals have quite a well-developed visual system for
dealing with details. For example, it has been shown that dogs possess quite a good visual
system that share many features with those of haplorhine primates~(\cite{10.1371/journal.pone.0090390}). 
A retinal region with a primate fovea-like cone photoreceptor density has been identified
but without the excavation of the inner retina. Similar anatomical structure observed in rare human subjects has been named fovea-plana. 
Basically, the results in~(\cite{10.1371/journal.pone.0090390}) challenge the
 dogma that within the phylogenetic tree of mammals, haplorhine primates with a fovea are the sole lineage in which the retina has a central bouquet of cones. 
In non-primate mammals, there is a central region of
specialization, called {\em area centralis}, which also is often located
temporal to the optic axis and demonstrates a local increase in
photoreceptor and retinal ganglion cell density
that plays a role somehow dual with respect to the fovea.
Like in  haplorhine primates, in those non-primate mammals we experiment 
focus of attention mechanisms that are definitely important from a functional viewpoint. 

%
% frogs' dilemma
%
This discussion suggests that the evolution of animals' visual system has followed many different paths
that, however, are related to focus of attention mechanisms, that are typically more effective for 
diurnal animals. There is, however, an evolution path which is definitely set apart, in which
the frog is most classic representer. 
More than sixty years ago, the visual behavior of the frog was posing an interesting
puzzle~(\cite{4065609}) which is mostly still on the table. In the words of the authors:
\begin{quote}{\small
The frog does not seem to see or, at any rate, is not concerned with the detail of 
stationary parts of the world around him. He will starve to death surrounded by food if it is not moving. 
His choice of food is determined only by size and movement.
}\end{quote}
No mammal experiments such a surprising behavior! However, the frog is not expected
to eat like mammals. When tadpoles hatch and get free, they attach themselves to plants 
in the water such as grass weeds, and cattails. 
They stay there for a few days and eat tiny bits of algae. 
Then the tadpoles release themselves from the plants and begin to swim freely, 
searching out algae, plants and insects to feed upon. At that time their visual system 
is ready. Their food requirements are definitely different from what mammals need
and their visual system has evolved accordingly for catching flying insects. 
%evolution in the visual system of amphybians~\cite{Dicke2009}
Interestingly, unlike mammals, the studies in~(\cite{4065609}) 
already pointed out that the frogs' retina is characterized by
uniformly distributed receptors with neither fovea nor {\em area centralis}.
Interestingly, this means that the frog does not focus attention by eye movements.
When the discussion focuses on functional issues the following natural questions
arise:
\begin{quote}
	{\bf Q7:} 
	{\em Why are the fovea and the area centralis convenient? 
	Why do primates and other animals focus attention, whereas 
	others, like the frog, do not?}
\end{quote}
%
 One can easily argue that any action that animals carry out 
needs to prioritize the frontal view.
On the other hand, this leads to the detriment of the peripheral vision, that 
is also very important. In addition, this could apply for the dorsal system whose
neurons are expected to provide information that is useful to support movements
and actions. Apparently, the ventral mainstream, with neurons 
involved in the ``what'' function, does not seem to benefit from foveate eyes.
Nowadays most successful computer vision models for object recognition, just like frogs, do not 
focus attention, since they carry out a uniform massive parallel computation on the
retina. Just like frogs, the cameras used in computer vision applications are uniformly
distributed, but machines seem to conquer human-like recognition capabilities 
on still images. Interestingly, unlike frogs, nowadays machines recognize quite well food 
properly served in a bowl.   This capabilities might be
due to the current strongly artificial  communication protocol. Machines benefit from supervised
learning of tons of supervised pairs, a process which, as already pointed out, cannot
be sustained in nature. 
On the other hand, as already pointed out, in order to attack the task of understanding 
what is located in a certain position, it is natural to think of  eyes based on fovea or on 
area centralis. The eye movements with the corresponding trajectory
of the focus of attention (FOA) is also clearly interwound with the temporal structure of 
video sources. 
%Its discussion opens the doors to an in-depth re-thinking of nowadays computer
%vision methods.
%From the theory proposed in this paper, the need
%of foveated retinas is strongly supported for achieving 
%efficient computation for the construction of visual features. 
%However, it will be argued that the most important reason for focussing attention is
%that of  dramatically simplifying the computation and limit the ambiguities 
%that come from the need to sustaining a parallel computation over each frame. \\
%When looking at Eq.~(\ref{ForthOrderDiff}) it becomes also clear that quick eye movements
%with respect to the dynamics of change of the weights of the filters dramatically
%simplifies the computation. 
%%% from Cutting the umbilical link 
%%% fovea
In particular, humans experiment eye movements when looking at fixed objects, 
which means that they continually experiment motion. Hence, also in case of fixed images, 
conjugate, vergence, saccadic, smooth pursuit, and vestibulo-ocular movements 
lead to acquire visual information from relative motion.  We claim that the 
production of such a continuous visual stream naturally drives
feature extraction,
%Rotation and scale invariances
%are likely to be somewhat artificial since, unlike motion invariance, 
%they cannot rely on continuous teaching from nature. 
%How does information on motion invariance arises? Suppose, again, we
%are moving your inch, and focus attention on the nail. Now, its features, which comes
%from its shape and color, are not expected to change as the nail is moving. The nail
%is the nail, regardless of its movement. 
since the corresponding convolutional filters, charged of representing features for
object recognition, are expected not to change during motion. 
The enforcement of this consistency condition creates a mine of visual data
during animal life! Interestingly, the same can happen for machines. 
Of course, we need to compute the optical flow at pixel level so as to enforce
the consistency of all the extracted features. Early studies 
on this problem~(see~\cite{HornAI1981}), along with recent related 
improvements (see e.g.~\cite{Baker:2011})
suggests to determine the velocity field by enforcing brightness invariance. 
As the optical flow is gained, it can be used to enforce motion consistency on the
visual features.
% Interestingly, the theory we propose is quite related to the
%variational approach that is used to determine the optical flow in~\cite{HornAI1981}.
%It is worth mentioning that an effective visual system must also develop 
%features that do not follow motion invariance. 
These features can be 
conveniently combined with those responsible of representing objects.
Early studies driven by these ideas are  reported in~\cite{DBLP:journals/cviu/GoriLMM16},
where the authors propose the extraction of visual features as a
constraint satisfaction problem, mostly based on information-based principles
and  early ideas on motion invariance. 
%%%% neuron model %%%%%%
\iffalse
This discussion suggests that neurons for feature extraction benefits from knowing the
position of the focus of attention. A layered structure with neurons associated with 
a certain position $x_{i}$ in the retina can conveniently be composed of neurons
where the classic convolutional structure is extended as follows:
%
\begin{equation}
	  \dot{\varphi}(x,t) = -
	  w(x-a)\varphi(x,t) +\sigma \bigg(\int w(x-a-z) u(z,t)\bigg)  
\end{equation}
%
\begin{equation}
	 g(x_{i}-a(t)) \dot{\varphi}(x_{i},t) = - w_{i,i}\varphi(x_{i},t) +\sigma \bigg(w_{i,\kappa} u(x_{\kappa},t))  + b_{i}(t)\bigg)  
\end{equation}
%
% w_{i,\kappa} non uniform ... depends on a(t)
%
Here, $\sigma(\cdot)$ is a sigmoidal function while the activation $\varphi$ is 
differentially accumulated and properly weighed by the bell-like function $g(\cdot)$.
Unlike classic neurons, the activation is driven by the position $a(x,t)$ of the focus of
attention that, on turn, depends also on the optical flow $v(x,t)$.
 \begin{figure}[H]
	\centering
	\includegraphics[width=5cm]{figs/NeuronModel.pdf}
\caption{\small Neuron model with activation reacting to the position of the focus of attention.
If the point $x_{i}$ where we compute the activation is far from the focus, the bell-shaped
function $g(\cdot)$ returns a vanishing term $g(x_{\kappa}-a)$, that leads the neuron to
keep its state. On the opposite, the more $x_{i}$ gets close to the focus of attention $a$, 
the higher is the convolutional contribution.}
\label{NeuronModel-Fig}
\end{figure}
\fi

%%%%%%%%%%%%%%%%%
The following remarks on focus of attention coming from nature seem to be important for conquering 
efficient visual skills for any intelligent agent.
Basically, it looks like we are faced with functional issues which mostly obeys 
information-based principles.
\begin{itemize}
\item {\em The FOA drives the definition of  visual primitives at pixel level. }\\
	The already mentioned visual skill that humans possess to perform pixel
	semantic labeling clearly indicates the capability of focusing on specific 
	points in the retina with high resolution.  Hence, FOA is needed if we want to 
	perform such a task.
\item	{\em Eye movements and FOA help estimating the probability distribution on the retina}\\
	At any time a visual agent clearly needs to possess a good estimation of the
	probability distribution over the pixels of the retina. This is important whenever 
	we consider visual tasks for which the position does matter. 
	This involves both the {\em where} and {\em what} neurons. In both cases
	it is quite obvious that any functional risk associated with the given task 
	should avoid reporting errors in regions of the retina where there is a uniform
	color. The probability distribution is of fundamental importance and it is definitely
	related to saliency maps built on focus of attention trajectories.
\item {\em FOA very well fits the need for receptive fields and deep nets}\\
	We have already discussed the marriage between receptive fields and deep
	networks. Interestingly, the FOA mechanisms emphasize the role of
	a single receptive field in the computational process that takes place at any
	time. The saccadic movements contribute to perform ``temporally segmented computations''
	over the retina on the different sequences produced by micro-saccadic movements.
	In addition, in~(\cite{Betti2018-CN-arxiv}), 
	the authors provide evidence of the fact that receptive fields do favor the
	development of biologically-plausible models based on local differential equations. 	
\item {\em Eye movements and FOA are the basis for establishing invariant laws.}\\
	The interplay between the FOA and the invariance properties is the 
	key for understanding human vision and general principles that drive 
	object recognition and scene interpretation. In order to understand the 
	nice circle that is established during the processes of learning in vision, 
	let us start exploring the very nature of eye movements in humans. 
	Basically, they produce visual sequences that are separated by saccadic
	movement, during which no information is acquired. 
	Interestingly, each of those sequences is composed  of pixels that
	somehow share common visual features. In case of micro-saccades 
	the corresponding micro-movements explore regions with a remarkable
	amount of details that are somehow characterized  by certain   features.
	The same holds true for smooth pursuit, where the invariance of the 
	extracted feature turns out to be a sort of primitive consistency property:
	objects do not change during their motion. 
	Hence, any visual feature associated with ``what neurons'' must be invariant 
	under any eye movement, apart from saccadic movements.
	Clearly, such an invariance has a truly unsupervised nature. 
	A deep net based on the discussed convolutional structure 
	 can in fact learn a set of latent features to be invariant
	under the FOA. This results in an impressive collection of 
	``labelled data'' that nature offers for free! 
	When thinking of the ``what'' neurons for which invariances need to be imposed,
	we can promptly realize that those which are close to the output are better suited
	for the enforcing of invariances. It is in fact quite obvious that for many
	of those invariances to take place we need a strong computational capability
	of the ``what neuron.'' Interestingly, this seems to suggest that ``where'' 
	neurons could better be located in the early layers of the hierarchy whereas
	``what'' neurons require higher abstraction. 
	
\item {\em FOA helps disambiguation at learning time}\\
	A puzzle is offered at learning time when two or more instance of the 
	same object are present in the same frame, maybe with different poses
	and scales. The FOA in this case helps disambiguating 
	the enforcement of  motion invariance. While the enforcement of weight sharing
	is ideal for directly implementing translation invariance, such a constraint
	doesn't facilitate other more complex invariances that can better be achieved
	by its removal. Basically the constraint of motion invariance under FOA movements
	naturally disambiguates the processing on different instances of the same 
	object since the computation takes place, at any time, on a single instance.	


\item {\em FOA drives the temporal interpretation of scene understanding}\\
	 The importance of FOA is not restricted to feature and object invariance,
	 since it involves also the interpretation of visual scenes. It is in fact the
	 way FOA is driven which sequentially selects the information 
	 for conquering the scene interpretation. Depending on the purpose of the
	 agent and on its level of scene understanding the FOA is consequently moved.
	This process clearly shows the fundamental role on the selection of the 
	points where to focus attention, an issue which is described in the following
	section. 
	 
\item {\em FOA helps disambiguating illusions}\\
	Depending on where an agent with foveate eyes focuses attention, 
	concepts that, strictly speaking, don't exist can emerge, thus originating
	an illusion. A noticeable example is  the 
	Kanizsa's triangle, but it looks like other illusions arise for 
	related reasons.  
	You can easily experiment that as you approach any detail, 
	it is perfectly perceived without any ambiguity. 
	A completion mechanism arises that leads us to perceive the
	 triangle  as soon as you move away from figure and the mechanism 
	is favored by focussing attention on the barycenter. 
	Interestingly, the different views coming from different points
	where  an agent with foveate eyes focuses attention 
	likely helps disambiguating illusions, a topic that
	has been recently studied in classic convolutional 
	networks~\cite{DBLP:journals/corr/abs-1903-01069,
	DBLP:conf/cogsci/BakerEKL18}.
\item {\em FOA helps facing the problem of ``concept drift''}\\ 
	When discussing motion invariance we mentioned the problem of concept drift.
	Clearly, this  could dramatically affect the practical implementation of the 
	motion invariance. However, amongst different types of FOA trajectories,
	the saccadic movements play the fundamental role of resetting the 
	process, which clearly faces directly problems of concept drift.	
\end{itemize}

The analysis on foveated-based neural computation nicely explains also the reason why 
humans cannot see video with a number of frames per second that exceeds the classic
sampling threshold. It turns out that this number is clearly connected with the velocity of the
scan paths of the focus of attention. Of course, this is a computational issue which
goes beyond biology and clearly affects machines as well. 

\begin{center}
\fbox{
\begin{minipage}{0.95\textwidth}\noindent \textit{
	{\bf Box 7:} The above items provide strong evidence on the 
	reasons why  foveate eyes turn out to be very effective for 
	scene understanding.
	Interestingly, we can export the information-based  principle of focussing attention
	to computer retinas by simulating eye movements. There is more: 
	machines could provide  multiple focuses  of attention which could 
	increase their visual skills significantly.
}\end{minipage}
}
\end{center}



\subsection{What drives eye movements?}
% perché movimento occhi e località (discussione lapo)
% il circolo di learning foa e riconosciemnto oggetti
Foveate animals need to move their eyes to properly focus attention. 
The previous discussion has emphasized the importance of performing appropriate
movements, which motivates the following question naturally arises:
\begin{quote}
{\bf Q8:} 
{\em 
What are the mechanisms that drive eye movements? 
}\end{quote}
Human eyes make jerky saccadic movements during ordinary visual 
acquisition.  One reason for these movements is that the fovea
provides high-resolution in portions of about $1,2$ degrees.
Because of such a small high resolution portions, the overall sensing of a scene
does require intensive movements of the fovea. Hence, the foveate movements
do represent a good alternative to eyes with uniformly high resolution 
retina. The information-based principles  discussed so far lead us to conclude that foveate
retinas with saccadic movements is in fact a solution that is 
computationally sustainable and very effective.
Fast reactions to changes in the surrounding visual environment require efficient attention mechanisms to reallocate computational resources to most relevant locations in the visual field. 
While current computational models keep improving their predictive ability thanks to the increasing availability of data, 
they are still far away from the effectiveness and efficiency exhibited by foveate animals. 
An in-depth investigation on biologically-plausible computational models of focus of attention 
that exhibit spatiotemporal locality is very important also for computer vision, where one
relies on parallel and distributed implementations. 
The research carried out by~(\cite{DBLP:journals/corr/abs-2006-11035}) suggests an 
interpretation based on a computational model where
attention emerges as a wave propagation process originated by visual stimuli corresponding to details and motion information. The resulting field obeys the principle of {\em inhibition of return},
so as not to get stuck in potential holes, and 
extend previous studies in~(\cite{DBLP:journals/pami/ZancaMG20}) with the main objective of providing 
spatiotemporal locality. In particular,  the idea of modeling the focus of attention by a gravitational process 
finds its evolution in the corresponding local model based on Poisson equation on the corresponding potential. 
Interestingly, Newtonian gravity yields an instantaneous propagation of signals, so as a sudden change in the mass density of a given pixel immediately affects the focus of attention, regardless of its location on the retina. 
These studies are driven by the principle that there are in fact sources which drive attention (e.g. masses in 
a gravitational field). At early cognitive stages,  attention mechanisms are mostly driven the presence of details
and movements.  This is the reason why the mentioned masses for modeling the focus of attention
have been based on the magnitude of the gradient of the brightness in the retina and on the optical flow. 
%
Interestingly, in children the mechanisms that drive  the focus of attention are strongly connected 
with the developmental stages. Newborns and children in their early stage only focus 
attention on details and movements and on a few recurrent visual patterns like faces. 
As time goes by, visual features conquer a semantic value and, consequently, the focus of attention
is gradually driven by specific intentions and corresponding plans. Of course, this is only possible 
after having acquired some preliminary capability of recognizing objects. Interestingly, as the
forward process that facilitate high level cognitive tasks from the focus of attention becomes effective
a corresponding backward process begins the improvement of the focus of attention. A
reinforcement loop is generated which is finalized to optimize the final purpose of the agent in
its own learning environment. 

 \begin{figure}[H]
	\centering
	\includegraphics[width=12cm]{figs/FOA.pdf}
\caption{\small Recognition is based on the  focus of attention. The generation of
the point of focus in the retina follows a development process. At early
stages, the ``gray'' blocks provides the inputs for the estimation of the focus
by extracting details and the optical flow. As time goes by, the recognition module
brings back information that makes it possible to improve the optical 
flow and the focus of attention by activating a constructive loop.}
\label{NeuronModel-Fig}
\end{figure}
\begin{center}
\fbox{
\begin{minipage}{0.95\textwidth}\noindent \textit{
	{\bf Box 8} Driving the focus of attention is definitely a crucial issue, simply because of its 
	already discussed fundamental role. We conjecture that this driving process 
	must undergo a developmental process, where we begins with details and 
	optical flow and prosegue with the fundamental feedback from the 
	environment which is clearly defined by the specific purpose of the agent.
}\end{minipage}
}
\end{center}
% dual nature of the mass and foa
\iffalse
\subsection{Why do we experiment illusions and visual generation?}
\begin{quote}
Causality and Non Rapid Eye Movements (NREM) sleep phases and visual generation (dreams)
\end{quote}
Computer vision is mostly based on huge training sets of images, whereas
humans use video streams for learning visual skills. Notice that because of 
the alternation of the biological rhythm of sleep, humans somewhat process collections of
visual streams pasted with relaxing segments composed of ``null'' video signal.
This happens mostly during NREM phases of sleep,
in which also eye movements and connection with visual memory 
are nearly absent. Interestingly, the
Rapid Eye Movements (REM) phase is, on the opposite, similar to ordinary 
visual processing, the only difference being that the construction of visual features
during the dream is based on the visual internal memory representations ~\cite{AndrillonNature2014}. 
As a matter of fact, the process of learning the filters experiments an alternation 
of visual information with the reset of the signal. 
%\marginnote{Day-night rhythm and relaxation of system dynamics.}
A good theory of learning visual features should provide evidence to claim that 
such a relaxation coming from the reset of the signal nicely fits  the 
purpose of optimizing an overall optimization index based on the 
previously stated principles. In particular, in~\cite{Betti2018-CN-arxiv}, the authors
point out that periodic resetting of the visual  information favors the optimization 
under causality requirements.
Hence, the role of eye movement and of sleep seem to be important 
for the optimal development of visual features. 
%In a sense, the theory offers a general framework for interpreting
%the importance of the day-night rhythm in the development of
%visual features. When combined with newborns blurring, it 
%contributes to a relaxation dynamical process that turns out to be
%of fundamental importance for the final purpose of optimization
%of the visual constraints. 
%
VISUAL GENERATION AND IMMAGINATION, DREAMS
??? Big pictures with the 10 questions which intersect the topics to investigate
(focus of attention, hierarchical structures, pixel primitives, continuity of time and 
gradual growth - boundary conditions) ...
??? Pelillo cite
\fi
\subsection{Why  is baby vision  blurred?}
\label{BlurringSection}
There are surprising results that come from developmental psychology 
on what a newborns see. Basically, their visual acuity grows gradually 
in early months of life. Interestingly,  Charles Darwin had already noticed
this very interesting phenomenon. In his words:
\begin{quote}
	{\bf Q9:} 
	{\small It was surprising how slowly he acquired the power of following with his eyes 
	an object if swinging at all rapidly; for he could not do this well when seven 
	and a half months old.}
\end{quote} 
At the end of the seventies, this early remark was given a technically sound
basis (see e.g.~\cite{DobsonVR-1978}).   In the paper, three techniques, --- optokinetic 
nystagmus (OKN), preferential looking (PL), and the visually evoked potential (VEP)--- were used to 
assess visual acuity in infants between birth and six months of age.
More recently,~(\cite{BraddickVR-2011}) provides 
an in-depth discussion on the state of the art in the field. It is clearly stated that 
for  newborns to gain adult visual acuity, depending on the specific visual test, 
several months are required. The following question naturally arises:
\begin{quote}
	{\em Why does it take 8-12 months for newborns to achieve adult visual acuity?
	Is the development of adult visual acuity a biological issue or does it come 
	from higher level computational laws of vision?}
\end{quote}
This pops up the discussion on the protection of the learning agent from
information overloading, which leads us to think of filtering the input
as stated by Eq.~(\ref{InputSmooth}). 
%
% Pelillo's criticisms - do I remove the part below?
%
The blurring of the video at early stage
of learning is compatible with a broader view of learning that, in addition to the 
involvement of the classic synaptic connections,  provides a direct ``simplification
of the input.''  At the beginning $\sigma=0$ and $\delta(x,0)=0$, which corresponds 
with the removal of the information. As time goes by $\sigma$ grows up and
it is supposed to approach the condition $\sigma=1$. Likewise, $\delta(x,t)$
yields the modification of the input at pixel level, so as it can grows up during the 
learning with the purpose of simplifying the task.
% However, the asymptotic
%condition which corresponds with the acquisition of the learning tasks 
%does require $\delta(x,t)$ for all pixels of the retina. 
Regardless of this specific input modification, the underlying idea is that
the process of learning consists of properly filtering the input with the
purpose of gradually acquiring the information. The development of any computation
model that adheres to this view is based on modifying the connections along with an
appropriate input filtering so as the learning agent always operates at an 
equilibrium point~(\cite{Betti2021-VB}).
%\begin{figure}[H]
%	\centering
%	\includegraphics[width=14cm]{figs/Blurring.pdf}
%\caption{Input blurring as the outcome of the joint learning in the weight space
%and in the input - plots from~(\cite{Betti2021-VB}).}
%\label{Blur-Fig}
%\end{figure}
%This paper provides evidence to conclude that the blurring process taking place
%in newborns is in fact a natural strategy to optimize the cognitive action defined
%by Eq.~\ref{CognitiveActionEq} under causality requirements.
%Moreover, the strict limitations both in terms of spatial and temporal resolution of the
%video signal, according to the theory, help conquering
%visual skills.  
\begin{center}
\fbox{
\begin{minipage}{0.95\textwidth}\noindent \textit{
	{\bf Box 9}: When promoting the role of time, the arising pre-algorithmic framework suggests
	extending the learning process to an appropriate modification of the input, that is
	finalized to achieve the  expected ``visual acuity'' at the end of the process of 
	learning. In doing so, one can think of generalization processes that are
	based on the convergence to fixed values of the weight connections, 
	but also on an opportune ``small perturbation'' of the input.
}\end{minipage}
}
\end{center}


\subsection{What is the interplay with language?}
The interplay of vision and language is definitely one of the most challenging
issues for an in-depth understanding of human vision. 
Along with the associated successes, 
the indisputable adoption of the supervised learning protocol in most challenging
object recognition problems caused the losing of motivations for an 
in-depth understanding of the way linguistic information is synchronized 
with visual clues. In particular, the way humans learn the  
name of objects is far away from the current formal supervised 
protocol. This can likely be better grasped when we begin considering that 
top level visual skills can be found in many animals (e.g. birds and primates), 
which clearly indicates that their acquisition is independent of language. 

Hence, as we clarify the interplay of vision and language we will 
likely address also the first question on how to  overcome the
the need for ``intensive artificial supervision.'' 
Since first linguistic skills arise in children when their visual acuity is already 
very well developed, there is a good chance that early simple
associations between objects and their names can easily be 
obtained by ``a few supervisions'' because of the very rich 
internal representation that has already been gained of those objects. 
It is in fact only a truly independent hidden representation of 
objects which makes it possible their subsequent association with 
a label! This seems to be independent of biology, whereas it looks 
like a fundamental information-based principle, which somehow
drives the development of ``what'' neurons. 

The interplay of language and vision has been recently very well 
addressed in a survey by~\cite{Lupyan_2012}).
 It is claimed that performance on tasks that have been presumed to be non-verbal is 
 rapidly modulated by language, thus rejecting  the distinction between verbal and non-verbal representations. While we subscribe the importance of sophisticated 
 interactions, we also reinforce the claim that capturing the identify of single objects
 is mostly a visual issue. However, when we move towards the acquisition of
 abstract notions of objects than the interaction with language is likely to be very important. 
 One needs to separate single objects coming in visual contexts with their
 own identity with respect to abstract notions of objects. We can see a specific 
 chair, but it's a different story to recognize that we have a chair in front of us. %qui

In Section~\ref{Focus-section} we addressed the issue of motion invariance
by claiming that it must properly be considered in the unified 
framework of focus of attention. We experiment eye movements 
either on still images or during motion. In the first case we can 
see micro-saccadic movements, whereas moving objects 
are properly tracked. While the enforcement of visual feature invariance
makes sense in both cases, there is a fundamental difference 
from an information-based viewpoint: The object tracking does provide
information on the object movement, so as one can propagate the
label to all the pixels that are connected with the pixel where we focus attention
by a non-vanishing optical flow. This conveys an enormous amount
of labelled information on the moving object and on its related segmentation.
There is more! While during micro-saccadic movements many invariant
features can be developed and it is not clear which one - if any - refers
to an explicit object as a whole, during smooth pursuit, thanks to the 
optical flow, the moving object, with its own label,  
provides an internal representation gained under this motion invariance
that is likely to be the secret for  bridging the linguistic attachment of labels to objects. 

The opportune exploitation of the optical flow in visual information
is of paramount importance for the evolution of theories of vision. 
In the last few years we have also seen a number of contributions
in  egocentric vision, where the assumption is that also the 
camera is moving. Interestingly, any sophisticated filtering of such
an external movement might neglect the importance of undergoing
developmental steps just like those that are fundamental for capturing
the interplay with language. Clearly, if you have already gained
good visual skills in object recognition, it is quite easy to check whether
you yourself are moving! 

Once again, the discussion carried out so far promotes the idea that 
for a visual agent to efficiently conquer the capabilities of recognizing
objects from a few supervisions, it must undergo some developmental steps
aimed at developing invariant representations of objects, so as
the actual linguistic supervision takes place only after the development of
those representations. But, when should we enable a visual agent to 
begin with the linguistic interaction? While one might address this question
when attacking the specific computational model under investigation, 
a more natural and interesting way to face this problem is to re-formulate the
question as:
\begin{quote}
	{\bf Q10:} 
	{\em
	How can we develop ``linguistic focusing mechanisms'' 
	that can drive the process of object recognition?}
\end{quote}
This  is done in a spectacular way in nature! 
Like vision, language development requires a lot of time. 
Interestingly, it looks like it requires more than vision. 
The discussion in Section~\ref{BlurringSection} indicates that the
gradual growth of the visual acuity is a possible clue to begin with
language synchronization. The discussed filtering process offers a protection from
visual information overloading that likely holds for language as well. 
As the visual acuity gradually increases, one immediately realizes
that the mentioned visual-language synchronization has a 
spatiotemporal structure. At a certain time, we need to inform
the agent on what we see at a certain position in the retina. 
An explicit implementation of such an association can be 
favored by an active learning process: the agent can ask itself
what is located at $(x,t)$. However, what if you 
cannot rely on such a precious active interactions?
For example, a linguistic description of the visual environment
is generally very sophisticated and mentions objects located in different
positions of the retina, without providing specific spatiotemporal information. 
Basically, this is a  sort of {\em weak supervision} that is 
more difficult to grasp. 
However, once again, developmental learning schemes can 
significantly help. At early stage of learning the agent's tasks can be 
facilitated by providing spatiotemporal information. For example, naming
the object located where the agent is currently focussing attention 
conveys information by a sort of human-like communication protocol.
As time goes by, the agent gains gradually the capability of recognizing
a few objects. What really matters is the confidence that is gained in 
such a task. When such a developmental stage is reached, linguistic 
descriptions and any sort of natural language based visual communication
can be conveniently used to reinforce the agent recognition confidence.
Basically, these weak supervisions turn out to be very useful since
they can profitably be attached where the agent  came up with a 
prediction that matches the supervision. 


\begin{center}
\fbox{
\begin{minipage}{0.95\textwidth}\noindent \textit{
	{\bf Box 10:} Computer vision and natural language processing have been mostly evolving independently
	one each other. While this makes sense, the time has come to explore the interplay
	between vision and language with the main purpose of going beyond the protocol of
	supervised learning for attaching labels to objects. 
	Interestingly challenges arises in scene interpretation when we begin considering 
	the developmental stages of vision that suggest gaining strong object invariance 
	before the attachment of linguistic labels.
}\end{minipage}
}
\end{center}

% reference suggested by Pelillo

\iffalse Pelillo\\
Si potrebbe obiettare che gli animali, a cui non si può attribuire un linguaggio evoluto come il nostro, hanno comunque sviluppato una capacità visiva come, se non migliore della nostra. D'altra parte una persona nata cieca sviluppa comunque capacità linguistiche normali.

Probabilmente, durante lo sviluppo, le due facoltà si aiutano l'un altra, ma non sembrerebbero essere necessarie l'una all'altra.

Ad ogni modo, la letteratura su percezione e linguaggio è vasta. Suggerisco di dare uno sguardo a questo articolo:

https://www.frontiersin.org/articles/10.3389/fpsyg.2012.00054/full
\fi








==> bk/EnPleinAir.tex <==
Posing the right questions is the first fundamental step to gain knowledge 
and solve problems. Hopefully, the questions raised  in this paper might give
you insights and contribute to face fundamental problems in computer vision. 
However, one might wonder what could be  the most concrete action for promoting
studies on the posed questions. So far, computer vision has  strongly benefited from the massive diffusion of
benchmarks which, by and large, are regarded as fundamental tools for performance evaluation.
However, it is clear that they are very well-suited to support the statistical machine learning
approach based on huge collections of labelled images. This paper, however, opens the doors 
to explore a different framework for performance evaluation. The emphasis on video instead of
images does not leads us to think of huge collection of video, but to a truly different approach
in which no collection at all is accumulated! Just like humans, machines are expected 
to live in their own visual environment. However, what is the scientific framework for 
evaluating the performance and understand when a theory carries out important new results?
Benchmark  bears some resemblance to the influential testing movement in psychology which has its roots in 
the turn-of-the-century work of Alfred Binet on IQ tests~(\cite{Binet1916}).
Both cases consist in attempts to provide a rigorous way of assessing the performance or the aptitude of a 
(biological or artificial) system, by agreeing on a set of standardized tests which, 
from that moment onward, become the ultimate criterion for validity. 
On the other hand, it is clear that the skills of any visual agent can be quickly evaluated 
and promptly judged by humans, simply by observing its behavior. 
Thus, we could definitely rely on  a {\em crowdsourcing performance evaluation scheme} 
where registered people can inspect and assess the performance of software agents 
~(\cite{DBLP:conf/iciap/GoriLMMP15}). 
We use the {\em term en plein air}  to  mimic the French Impressionist painters of the 19th-century and, more 
generally, the act of painting outdoors. This term suggests that visual agents should be evaluated 
by allowing people to see them in action, virtually opening the doors of research labs. 
The en plein air proposal allows others to test our algorithms and to contribute to this 
evaluation method by providing their own data, their own results, or the comparisons with their 
own algorithms. 

While the idea of shifting computer vision challenges into the wild will deserves attention 
one cannot neglect the difficulties that arise from the lack of a truly lab-like environment
for supporting the experiments. The impressive progress in computer graphics, however, 
is offering a very attractive alternative that can dramatically facilitate the developments 
of approaches to computer vision that are based on the on-line treatment of the 
video (see e.g.~\cite{DBLP:journals/corr/abs-2007-08224}).

%\begin{center}
%\fbox{
%\begin{minipage}{0.95\textwidth}\noindent \textit{
	Needless to say, computer vision has been fueled by the availability of huge labelled 
	image collections, which clearly shows that fundamental role played by 
	pioneer projects in this direction (see e.g.~\cite{imagenet_cvpr09}).
	The ten questions posed in this paper will likely be better addressed only when 
	scientists will put more emphasis on the en plein air environment. In the 
	meantime, the major claim of this paper is that the experimental setting 
	needs to move to virtual visual environments. Their photorealistic level along
	with explosion of the generative capabilities make these environment just
	perfect for a truly new performance evaluation of computer vision. The 
	advocated crowdsourcing approach might really change the way we measure
	the progress of the discipline.
%}\end{minipage}
%}
%\end{center}


==> bk/EnPleinAir_2.tex <==
\section{The ``en plain air'' perspective}
\label{APA-sec}
Posing the right questions is the first fundamental step to gain knowledge 
and solve problems. Hopefully, the questions raised  in this paper might give
you insights and contribute to face fundamental problems in computer vision. 
However, one might wonder what could be  the most concrete action for promoting
studies on the posed questions. So far, computer vision has  strongly benefited from the massive diffusion of
benchmarks which, by and large, are regarded as fundamental tools for performance evaluation.
However, it is clear that they are very well-suited to support the statistical machine learning
approach based on huge collections of labelled images. This paper, however, opens the doors 
to explore a different framework for performance evaluation. The emphasis on video instead of
images does not leads us to think of huge collection of video, but to a truly different approach
in which no collection at all is accumulated! Just like humans, machines are expected 
to live in their own visual environment. However, what is the scientific framework for 
evaluating the performance and understand when a theory carries out important new results?
Benchmark  bears some resemblance to the influential testing movement in psychology which has its roots in 
the turn-of-the-century work of Alfred Binet on IQ tests~(\cite{Binet1916}).
Both cases consist in attempts to provide a rigorous way of assessing the performance or the aptitude of a 
(biological or artificial) system, by agreeing on a set of standardized tests which, 
from that moment onward, become the ultimate criterion for validity. 
On the other hand, it is clear that the skills of any visual agent can be quickly evaluated 
and promptly judged by humans, simply by observing its behavior. 
Thus, we could definitely rely on  a {\em crowdsourcing performance evaluation scheme} 
where registered people can inspect and assess the performance of software agents 
~(\cite{DBLP:conf/iciap/GoriLMMP15}). 
We use the {\em term en plein air}  to  mimic the French Impressionist painters of the 19th-century and, more 
generally, the act of painting outdoors. This term suggests that visual agents should be evaluated 
by allowing people to see them in action, virtually opening the doors of research labs. 
The en plein air proposal allows others to test our algorithms and to contribute to this 
evaluation method by providing their own data, their own results, or the comparisons with their 
own algorithms. 

While the idea of shifting computer vision challenges into the wild will deserves attention 
one cannot neglect the difficulties that arise from the lack of a truly lab-like environment
for supporting the experiments. The impressive progress in computer graphics, however, 
is offering a very attractive alternative that can dramatically facilitate the developments 
of approaches to computer vision that are based on the on-line treatment of the 
video (see e.g.~\cite{DBLP:journals/corr/abs-2007-08224}).

%\begin{center}
%\fbox{
%\begin{minipage}{0.95\textwidth}\noindent \textit{
	Needless to say, computer vision has been fueled by the availability of huge labelled 
	image collections, which clearly shows that fundamental role played by 
	pioneer projects in this direction (see e.g.~\cite{imagenet_cvpr09}).
	The ten questions posed in this paper will likely be better addressed only when 
	scientists will put more emphasis on the en plein air environment. In the 
	meantime, the major claim of this paper is that the experimental setting 
	needs to move to virtual visual environments. Their photorealistic level along
	with explosion of the generative capabilities make these environment just
	perfect for a truly new performance evaluation of computer vision. The 
	advocated crowdsourcing approach might really change the way we measure
	the progress of the discipline.
%}\end{minipage}
%}
%\end{center}


==> bk/Introduction.tex <==
\vspace{-3cm}
%  
% object identity, abstract object notion, actions, affordance, 
%


While the emphasis on a general theory of vision was already 
the main objective at the dawn of the discipline~\cite{Marr82}, it has evolved without a systematic exploration of foundations in machine learning. When the target is moved to unrestricted visual environments and the emphasis is shifted from huge labelled databases to a human-like protocol of interaction, we need to go beyond the current peaceful interlude that we are experimenting in vision and machine learning. A fundamental question a good theory is expected to answer is why children can learn to recognize objects and actions from a few supervised examples, whereas nowadays supervised learning approaches strive to achieve this task. In particular, why are they so thirsty for supervised examples? Interestingly, this fundamental difference seems to be deeply rooted in the different communication protocol at the basis of the acquisition of visual skills in children and machines. 

%%%%%%%%%%%%%%%
% video instead of images
%%%%%%%%%%%%%%%
So far, the semantic labeling of pixels of a given video has been mostly carried out at frame level. This seems to be the natural outcome of a very well-established tradition in pattern recognition methods working on images, which have given rise to nowadays emphasis on collecting big labelled image databases (e.g.~\cite{imagenet_cvpr09}) 
with the purpose of devising and testing challenging machine learning algorithms. While this framework is the one in which most of nowadays state of the art object recognition approaches have been developing, we argue that there are strong arguments to start exploring the more natural visual interaction that animals experiment in their own environment. 

%\marginnote{Learning in wild visual environments.}
Basically, we need to process video instead of image collection,
which could naturally led to a paradigm-shift
in the associated processes of learning to see. The idea of shifting to video is very much 
related to the growing interest of {\em learning in the wild} that has been explored in the
last few years\footnote{See. e.g.~\url{https://sites.google.com/site/wildml2017icml/}.}.
The learning processes that take place in this kind of environments have a different
nature with respect to those that are typically considered in machine learning. 
Learning convolutional nets on ImageNet typically consists of updating the weights
from the processing of temporally unrelated images, whereas a video carries out
information that is characterized by a smooth changes from close frames. 
While ImageNet is a collection of unrelated images, a video supports information
only when motion is involved. In presence of fixed images that last for awhile, the corresponding stream of equal frames basically supports only the information 
of a single image.
As a consequence, it is clear that visual environments diffuse information only when
motion is involved. There is no transition from one image to the next one ---like in
ImageNet--- but, as time goes by, the information is only carried out by motion,
which modifies one frame to the next one according to the optical flow. Once we 
deeply capture this fundamental features of visual environment, we early realize that
we need a different theory of machine learning that must be capable of
naturally processing streams instead of a collection of independent images.   


%%%%%%%%%%%%%%%
% motion invariance
%%%%%%%%%%%%%%%
A crucial problem that was recognized by Poggio and Anselmi~\cite{Poggio:2016:VCD} is the need to incorporate visual invariances
into deep nets, which goes well beyond the simple translation invariance 
that is currently characterizing
convolutional networks. They propose an elegant mathematical framework 
on visual invariance and enlighten some intriguing neurobiological connections. 
Overall, the ambition of extracting distinctive features from vision poses a challenging 
problem. While in the literature we have been typically concerned with feature extraction that is independent of classic geometric transformation, it looks like we are still missing the fantastic human skill of capturing distinctive features that we can see when
recognizing ironed and rumpled shirts! There is no apparent difficulty to recognize shirts by keeping the recognition coherence in case we roll up the sleeves, or we simply curl them up into a ball for the laundry basket. Of course, there are neither rigid transformations, like translations and rotation, nor scale maps that transforms an ironed shirt into the same shirt thrown into the laundry basket. 
Is there any natural invariance?

In this book, we claim that
motion invariance is in fact the only one that we need.
%\marginnote{The paradigm-shift of motion invariance}
Translation,  scale, and rotation invariances, 
that have been the subject of many studies, are in
fact instances of invariances that can be fully gained whenever we develop the 
ability to detect features that are invariant under motion. 
If my inch moves closer and closer to my eyes then any of its representing features 
that is motion invariant will also be scale invariant. The
finger will become bigger and bigger as it approaches my face, but it is still my inch!
Clearly, translation, rotation, and complex deformation invariances  derive from
motion invariance. Humans life always experiments motion, so as the gained visual
invariances naturally arise from motion. Animals with foveal eyes also
move quickly the focus of attention when looking at fixed objects, which means that they
continually experiment motion. Hence, also in case of fixed images, 
conjugate, vergence, saccadic, smooth pursuit, and vestibulo-ocular movements lead to acquire visual information from relative motion.  We claim that the 
production of such a continuous visual stream naturally drives
feature extraction,
%Rotation and scale invariances
%are likely to be somewhat artificial since, unlike motion invariance, 
%they cannot rely on continuous teaching from nature. 
%How does information on motion invariance arises? Suppose, again, we
%are moving your inch, and focus attention on the nail. Now, its features, which comes
%from its shape and color, are not expected to change as the nail is moving. The nail
%is the nail, regardless of its movement. 
since the corresponding convolutional filters, charged of representing features for
object recognition, are expected not to change during motion. 
The enforcement of this consistency condition creates a mine of visual data
during animal life. Interestingly, the same can happen for machines. 
Of course, we need to compute the optical flow at pixel level so as to enforce
the consistency of all the extracted features. Early studies 
on this problem~\cite{HornAI1981}, along with recent related 
improvements (see e.g.~\cite{Baker:2011})
suggests to determine the velocity field by enforcing brightness invariance. 
As the optical flow is gained, it can be used to enforce motion consistency on the
visual features.
% Interestingly, the theory we propose is quite related to the
%variational approach that is used to determine the optical flow in~\cite{HornAI1981}.
It is worth mentioning that an effective visual system must also develop 
features that do not follow motion invariance. These features can be 
conveniently combined with those responsible of representing objects.
Early studies driven by these ideas are  reported in~\cite{DBLP:journals/cviu/GoriLMM16},
where the authors propose the extraction of visual features as a
constraint satisfaction problem, mostly based on information-based principles
and  early ideas on motion invariance. 

%%\marginnote{Learning as the minimization of the cognitive action.}
%In this paper, the importance of motion invariance is stressed and, moreover,
%the solution is derived in the framework of the principle of 
%cognitive action~\cite{DBLP:journals/tcs/BettiG16}, which gives rise  to a
%time-variant differential equation, where the Lagrangian coordinates
%corresponds with the values of the convolutional filters. 
%It is pointed out that, under causality conditions, the well-position
%of the problems arises thanks to the process of video-blurring taking
%place at the beginning of learning, which has also been experimented
%in children. 
%The learning process can be interpreted in the framework of the minimization
%of the cognitive action that offers a self-consistent framework. In particular, if the video signal is almost periodic~\cite{besicovitch1954almost},
%then the computational model reduces to an asymptotically stable 
%differential equation that yields a sort of statistical consistency. 

In this book we mostly deal with a discussion of the principles that
one should follow to construct a sound theory of vision that, later on, can 
likely be also applied to computer vision. In addition, we discuss some of the
reasons of the limitations of current approaches, where perceptual and linguistic
tasks interwound with vision are not properly covered. This issue is enlighten 
by proposing a hierarchy of cognitive tasks connected with vision that contributes
to shed light on the intriguing connection between gaining perceptual and linguistic
skills.  The discussion suggests that most problems
of computer vision are likely to be posed according to the historical evolution of
the applications more than on an in-depth analysis of the underlying computational
processes. While this choice has been proven to be successful in many real-world
cases, stressing this research guideline might led, on the long run, to wrong directions. 

% eye movements and citation to nips

==> bk/Introduction_2.tex <==
%%%% Prologue %%%%
%\subsection{Prologue}
The professional construction of huge supervised visual 
data bases has significantly contributed to the spectacular 
performance of deep learning. However, the extreme exploitation 
of the truly artificial communication protocol of supervised learning 
has been experimenting its drawbacks, including the vulnerability
to adversarial attacks, which might also be tightly connected to the
negligible role typically played by  the temporal structure.
Aren't we missing something?  It looks like Nature did a great job by using time to ``sew all the video frames'', whereas it  goes unnoticed to our eyes!  
At the dawn of pattern recognition, when we also began to cultivate the
idea of interpreting natural video, in order to simplify the problem 
of dealing with a huge amount of information we removed time, the connecting thread between frames, and began playing with 
the pattern regularities that emerge at the spatial level. As a consequence, all
tasks of pattern recognition were turned into problems
formulated on  collections of images, where 
the crucial role of temporal coherence was neglected. 
Interestingly, when considering the general problem of object recognition
and scene interpretation, the joint role of the computational resources and the access to huge visual databases of supervised data has 
contributed to erect nowadays
``reign of computer vision''.  
At a first glance this is reasonable, especially if you consider that video were
traditionally heavy data sources  to be played with. 
However, a closer look reveals that 
we are in fact neglecting a fundamental clue to interpret visual information, 
and that we have ended up into problems where the extraction of the visual concepts is mostly based on  spatial  regularities.
On the other hand, reigns have typically consolidated rules from which it's hard to escape.  This is common in novels and real life.
``The Three Princes of Serendip'' is the English version of ``Peregrinaggio di tre giovani figliuoli del re di Serendippo,'' published by Michele Tramezzino in Venice on 1557. These princes journeyed widely, and as they traveled they continually made discoveries, by accident and sagacity, of things they were not seeking. A couple of centuries later, in a letter of January 28, 1754 to a British envoy in Florence, the English politician and writer Horace Walpole coined a new term: serendipity, which is succinctly characterized as the art of finding something when searching for something else. Couldn't similar travels open new
scenario in computer vision? Couldn't the visit to 
well-established scientific domains, where time is dominating the scene, 
open new doors to an in-depth understanding of vision? 
We need to stitch the frames to recompose the video using time as a thread, the same thread we had extracted to work on the images at the birth of the discipline.
We need to go beyond a peaceful interlude and think of 
learning theories based on video more than on images!
%%%%%%%

This paper is a travel towards the frontiers of the science of vision with special emphasis
to object perception. We drive the discussion by a number
of  curios questions that mostly arise
as one tries to interpret and disclose natural vision processes 
in a truly computational framework. Unfortunately, as yet, we are far away
from addressing the posed questions. However, this paper comes from the 
awareness that posing right questions on the discipline might themselves stimulate 
its progress. 


\section{Cutting the umbilical cord with pattern recognition}
\label{Unbilicalsec}
%%% Roli's comments 
In the eighties, Satosi Watanabe wrote a seminal book~(\cite{10.5555/4394}) 
in which he early pointed out the different facets of pattern recognition that
can be regarded as  perception, categorization,  induction, pattern recognition,
as well  as statistical decision making.
Most of the modern work on computer vision for object perception fits with 
Watanabe's view of pattern recognition as statistical decision making and pattern recognition as categorization.
%
Based on optimization schemes with billions of variables and universal  
approximation capabilities, the spectacular results of deep learning have elevated 
this view of pattern recognition to a position where it is hardly debatable. 
While the emphasis on a general theory of vision was already 
the main objective at the dawn of the discipline~(\cite{Marr82}), 
its evolution has been mostly marked to significant experimental achievements. 
Most successful approaches  seem to be the natural outcome of a very well-established tradition in pattern recognition methods working on images, which have given rise to nowadays emphasis on collecting big labelled image databases (e.g.~\cite{imagenet_cvpr09}).

%
% epistemological issue
%
However, in spite of these successful results, this could be the time of an in-depth rethinking of what we have 
been doing, especially by considering the remarkable traditions of the 
overall field of vision.  In his seminal book,
Freeman J. Dyson~(\cite{dyson2004infinite}),  discusses two distinct styles of scientific thinking: unifying and diversifying. He claimed that most sciences are dominated by one or the other in various periods of their history. Unifiers are people whose driving passion is to find general principles, whereas 
Diversifiers are people with the passion of details. 
Historical progress of science is often a blend of unification and diversification. 
Couldn't it be the right time to exploit the impressive literature in the field vision
to conquer a more unified view of object perception? 

%
% Cognitive Ethology
%

In the last few years, a number of studies in psychology cognitive science have 
been pushing truly novel
approaches to vision. In~(\cite{Kingstone2010}), it is pointed out that 
a critical problem that continues to bedevil the study of human cognition is related to 
the  remarkably successes gained in experimental psychology, where 
one is typically involved in simplifying
the experimental context  with the purpose to discover causal relationships. 
In so doing we minimize the complexity of the environment and maximize the experimental control,
which is typically done also in computer vision when we face object recognition. 
However, one might ask whether such a simplification is really adequate and, most
importantly, if it is indeed a simplification. Are we sure that treating vision as a collection
of unrelated frames leads to simplification of learning visual tasks? 
In this paper we argue this not the case, since 
cognitive processes vary substantially with changes in context. 
When promoting the actual environmental interaction,~\cite{Kingstone2010}
introduce a novel research approach, called, ``Cognitive Ethology'', 
where one opts to explore first how people behave in a truly naturally situation. 
Once we have collected experience and evidence in the actual environment then 
we can move into the laboratory to test hypotheses.  This strongly suggests
that also machines should learn in the wild!

%
% vision as action ... in addition to vision as perception
%

Other fundamental lessons come from the school of robotics
for whatever involves the control of object-directed actions. 
In~(\cite{Ballard2011}), it is pointed out that 
``the purpose of vision is very different when looking at a static scene to when engaging in real-world behavior.''  The interplay between  extracting visual information and coordinating the motor actions 
is a crucial issue to face for gaining an in-depth understanding of vision.  
One early realizes that manipulation of objects is not something
that we learn from a picture; it looks like you definitely need to act yourself if you want to 
gain such a skill. Likewise, the perception of the objects you manipulate 
can nicely get a reinforcement form such a mechanical feedback.
The mentioned interplay between perception and action finds an
intriguing convergence in the natural processes of gaze control and, overall, on 
the focus of attention~(\cite{DBLP:journals/ai/Ballard91}).
It looks like  {\em animate vision} goes beyond passive information extraction
and plays an important role in better posing most vision tasks.

%
% predictive coding
%
The studies in computer vision might benefit significantly also from the exploration of
the links with predictive coding~\cite{rao:natneuro99} that have had a remarkable impact in neuroscience.
In that framework one is willing to study theories of brain in which it constantly generates and updates a ``mental model''
of the environment. Overall, the model is supposed  to generate its own predictions of sensory input and 
compare them to the actual sensory input. The prediction error is expected to be used to update and revise the mental model.
While most of the studies in deep learning have been focused on the direct learning of object categories, 
there are a few contributions also in the direction of performing a sort of predictive coding by 
means of auto-encoding architectures~(\cite{DBLP:journals/corr/RonnebergerFB15}).
This neural network, which is referred to as an {\em U-net}, is used for medical image segmentation. 


\section{Dealing with video instead of images}
While the emphasis on methods rooted on still images is common on  most of nowadays 
state of the art object recognition approaches, in this paper we argue
 that there are strong arguments to start exploring the more natural visual interaction 
 that animals experiment in their own environment. 
The idea of shifting to video is very much 
related to the growing interest of {\em learning in the wild} that has been explored in the
last few years\footnote{See. e.g.~\url{https://sites.google.com/site/wildml2017icml/}.}.
The learning processes that take place in this kind of environments have a different
nature with respect to those that are typically considered in machine learning. 
%Learning convolutional nets on ImageNet typically consists of updating the weights
%from the processing of temporally unrelated images, whereas a video carries out
%information that is characterized by a smooth changes from close frames. 
While ImageNet~(\cite{imagenet_cvpr09}) is a collection of unrelated images, a video supports information only when motion is involved. In presence of still images that last for awhile, the
 corresponding stream of equal frames only conveys the information of a single image
 - apart from the duration of the interval in which the video has been kept constant. 
As a consequence,  visual environments mostly diffuse information only when
motion is involved. As time goes by, the information is only carried out by motion,
which modifies one frame to the next one according to the optical flow. Once we 
deeply capture this fundamental feature of vision,
we realize that a different theory of machine learning is needed that must be 
capable of naturally processing streams instead of a collection of independent images.   

%%\marginnote{Learning as the minimization of the cognitive action.}
%In this paper, the importance of motion invariance is stressed and, moreover,
%the solution is derived in the framework of the principle of 
%cognitive action~\cite{DBLP:journals/tcs/BettiG16}, which gives rise  to a
%time-variant differential equation, where the Lagrangian coordinates
%corresponds with the values of the convolutional filters. 
%It is pointed out that, under causality conditions, the well-position
%of the problems arises thanks to the process of video-blurring taking
%place at the beginning of learning, which has also been experimented
%in children. 
%The learning process can be interpreted in the framework of the minimization
%of the cognitive action that offers a self-consistent framework. In particular, if the video signal is almost periodic~\cite{besicovitch1954almost},
%then the computational model reduces to an asymptotically stable 
%differential equation that yields a sort of statistical consistency. 
%In this paper we mostly deal with a discussion of the principles that
%one should follow to construct a sound theory of vision that, later on, can 
%likely be also applied to computer vision. In addition, we discuss some of the
%reasons of the limitations of current approaches, where perceptual and linguistic
%tasks interwound with vision are not properly covered. This issue is enlighten 
%by proposing a hierarchy of cognitive tasks connected with vision that contributes
%to shed light on the intriguing connection between gaining perceptual and linguistic
%skills.  The discussion suggests that 

% eye movements and citation to nips
%\section{Cutting the umbilical cord with pattern recognition}
The scientific communities of pattern recognition and computer vision
have a longstanding tradition of strong intersections. 
As the notion of pattern began to circulate at the end of the 
Fifties, the discipline of pattern recognition grew up quickly
around the notion of pattern. No matter what kind of representation a
pattern is given, its name  conveys the  underlining assumption that,
regardless of the way they are obtained,
the recognition process involves single patterns. 
It is in fact their accumulation in appropriate collections which 
gives rise to statistical machine learning. 
While computer vision can hardly be delimited in terms both  of
methodologies and applications, the dominant foundations are
still the same promoted by the pioneers of pattern recognition.  
Surprisingly enough, there is no much attention on the crucial
role of the position (pixel) on which the decision is carried out
and, even more, the role of time in the recognition processes
doesn't seem to play a central role. 
It looks like we are mostly ignoring  that we are in front of
spatiotemporal information, whose reduction to isolated patterns
might not be a natural solution especially for the complex tasks
that we have been recently tackling. 

%\section{The long-standing tradition of pattern recognition}

%\subsection{The segmentation-recognition chicken-egg  dilemma}
In the last decades, the massive production of electronic documents,
along with their printed version, 
has given rise to specialized software tools to extract textual information
from optical data. Most optical documents, like 
tax forms or invoices, are characterized by a certain layout which
dramatically simplifies the process of information extraction. 
Basically, as one recognizes the class of a document, its layout
offers a significant prior on what we can expect to find in its
different areas. For those documents, the segmentation process 
can often be given a somewhat formal description, so as most of the problems are
reduced to deal with the presence of noise. As a matter of 
fact, in most real-world problems, the noise doesn't compromise
significantly the presence of segmentation, that is very well driven
by the expectations provided in each pixel of the documents.
These guidelines have been fueling the field of documental analysis
and recognition (DAR), whose growth in the last few years has led to
impressive results~(\cite{DBLP:journals/pami/MarinaiGS05}). 
Unfortunately, in most real-world problems, as we move to natural images and vision,
the methodology used in DAR is not really effective in most challenging problems.
The reason is that there is no longer a reliable anchor
to which one can cling for segmenting the objects 
of a scene. While we can provide a clear description of chars and 
lines in optical documents, the same doesn't hold for the picture
of a car which is mostly hidden by a truck during the overtaking. 
Humans exhibit a spectacular detection ability 
by simply relying on  small glimpses at different scale and 
rotations. In no way those a cognitive processes are reducible to
the well-posed segmentation problems of chars and lines in optical documents.
As we realize that there is a car, we can in fact provide its segmentation.
Likewise, if an oracle gives us the segmented portion of a car,
we can easily classify it. Interestingly, we don't really know 
which of the two processes is given a priority - if any. 
We are trapped into the chicken-egg dilemma on whether 
classification of objects must take place first of segmentation or vice versa.
Amongst others, this issue has been massively investigated by
in~(\cite{DBLP:conf/eccv/BorensteinU02})
and early pointed out in~(\cite{UllmanShimon1979Tiov}).
This intriguing dilemma might be connected with the 
absence of  focus of attention,
which necessarily leads to holistic mechanisms of information extraction.
Unfortunately, while holistic mechanisms are required at a certain level of abstraction, 
the segmentation is a truly local process that involves
low level features.
%Basically, there is no decoupling between the visual source and its linguistic description.  

The bottom line is that most problems
of computer vision are are posed according to the historical evolution of
the applications more than on an in-depth analysis of the underlying computational
processes. While this choice has been proven to be successful in many real-world
cases, stressing this research guideline might led, on the long run, 
to sterile directions. 
%%%%%%%%%%%%%%%
% invariances in the literature
%%%%%%%%%%%%%%%
Somewhat outside the mainstream of massive exploration of supervised 
learning, Poggio and Anselmi~(\cite{Poggio:2016:VCD}) pointed out the 
crucial role of incorporating appropriate visual invariances
into deep nets to go beyond the simple translation invariance 
that is currently characterizing convolutional networks. They propose an elegant mathematical framework 
on visual invariance and enlighten some intriguing neurobiological connections. 
Couldn't it be the case that the development of appropriate invariances is exactly what 
we need to go one step beyond?




==> bk/Introduction_3.tex <==
%%%% Prologue %%%%
%\subsection{Prologue}
The professional construction of huge supervised visual 
data bases has significantly contributed to the spectacular 
performance of deep learning. However, the extreme exploitation 
of the truly artificial communication protocol of supervised learning 
has been experimenting its drawbacks, including the vulnerability
to adversarial attacks, which might also be tightly connected to the
negligible role typically played by  the temporal structure.
Aren't we missing something?  It looks like Nature did a great job by using time to ``sew all the video frames'', whereas it  goes unnoticed to our eyes!  
At the dawn of pattern recognition, when we also began to cultivate the
idea of interpreting natural video, in order to simplify the problem 
of dealing with a huge amount of information we removed time, the connecting thread between frames, and began playing with 
the pattern regularities that emerge at the spatial level. As a consequence, all
tasks of pattern recognition were turned into problems
formulated on  collections of images, where 
the crucial role of temporal coherence was neglected. 
Interestingly, when considering the general problem of object recognition
and scene interpretation, the joint role of the computational resources and the access to huge visual databases of supervised data has 
contributed to erect nowadays
``reign of computer vision''.  
At a first glance this is reasonable, especially if you consider that video were
traditionally heavy data sources  to be played with. 
However, a closer look reveals that 
we are in fact neglecting a fundamental clue to interpret visual information, 
and that we have ended up into problems where the extraction of the visual concepts is mostly based on  spatial  regularities.
On the other hand, reigns have typically consolidated rules from which it's hard to escape.  This is common in novels and real life.
``The Three Princes of Serendip'' is the English version of ``Peregrinaggio di tre giovani figliuoli del re di Serendippo,'' published by Michele Tramezzino in Venice on 1557. These princes journeyed widely, and as they traveled they continually made discoveries, by accident and sagacity, of things they were not seeking. A couple of centuries later, in a letter of January 28, 1754 to a British envoy in Florence, the English politician and writer Horace Walpole coined a new term: serendipity, which is succinctly characterized as the art of finding something when searching for something else. Couldn't similar travels open new
scenario in computer vision? Couldn't the visit to 
well-established scientific domains, where time is dominating the scene, 
open new doors to an in-depth understanding of vision? 
We need to stitch the frames to recompose the video using time as a thread, the same thread we had extracted to work on the images at the birth of the discipline.
We need to go beyond a peaceful interlude and think of 
learning theories based on video more than on images!
%%%%%%%

This paper is a travel towards the frontiers of the science of vision with special emphasis
to object perception. We drive the discussion by a number
of  curios questions that mostly arise
as one tries to interpret and disclose natural vision processes 
in a truly computational framework. Unfortunately, as yet, we are far away
from addressing the posed questions. However, this paper comes from the 
awareness that posing right questions on the discipline might themselves stimulate 
its progress. 


\section{Cutting the umbilical cord with pattern recognition}
\label{Unbilicalsec}
%%% Roli's comments 
In the eighties, Satosi Watanabe wrote a seminal book~(\cite{10.5555/4394}) 
in which he early pointed out the different facets of pattern recognition that
can be regarded as  perception, categorization,  induction, pattern recognition,
as well  as statistical decision making.
Most of the modern work on computer vision for object perception fits with 
Watanabe's view of pattern recognition as statistical decision making and pattern recognition as categorization.
%
Based on optimization schemes with billions of variables and universal  
approximation capabilities, the spectacular results of deep learning have elevated 
this view of pattern recognition to a position where it is hardly debatable. 
While the emphasis on a general theory of vision was already 
the main objective at the dawn of the discipline~(\cite{Marr82}), 
its evolution has been mostly marked to significant experimental achievements. 
Most successful approaches  seem to be the natural outcome of a very well-established tradition in pattern recognition methods working on images, which have given rise to nowadays emphasis on collecting big labelled image databases (e.g.~\cite{imagenet_cvpr09}).

%
% epistemological issue
%
However, in spite of these successful results, this could be the time of an in-depth rethinking of what we have 
been doing, especially by considering the remarkable traditions of the 
overall field of vision.  In his seminal book,
Freeman J. Dyson~(\cite{dyson2004infinite}),  discusses two distinct styles of scientific thinking: unifying and diversifying. He claimed that most sciences are dominated by one or the other in various periods of their history. Unifiers are people whose driving passion is to find general principles, whereas 
Diversifiers are people with the passion of details. 
Historical progress of science is often a blend of unification and diversification. 
Couldn't it be the right time to exploit the impressive literature in the field vision
to conquer a more unified view of object perception? 

%
% Cognitive Ethology
%

In the last few years, a number of studies in psychology cognitive science have 
been pushing truly novel
approaches to vision. In~(\cite{Kingstone2010}), it is pointed out that 
a critical problem that continues to bedevil the study of human cognition is related to 
the  remarkably successes gained in experimental psychology, where 
one is typically involved in simplifying
the experimental context  with the purpose to discover causal relationships. 
In so doing we minimize the complexity of the environment and maximize the experimental control,
which is typically done also in computer vision when we face object recognition. 
However, one might ask whether such a simplification is really adequate and, most
importantly, if it is indeed a simplification. Are we sure that treating vision as a collection
of unrelated frames leads to simplification of learning visual tasks? 
In this paper we argue this not the case, since 
cognitive processes vary substantially with changes in context. 
When promoting the actual environmental interaction,~\cite{Kingstone2010}
introduce a novel research approach, called, ``Cognitive Ethology'', 
where one opts to explore first how people behave in a truly naturally situation. 
Once we have collected experience and evidence in the actual environment then 
we can move into the laboratory to test hypotheses.  This strongly suggests
that also machines should learn in the wild!

%
% vision as action ... in addition to vision as perception
%

Other fundamental lessons come from the school of robotics
for whatever involves the control of object-directed actions. 
In~(\cite{Ballard2011}), it is pointed out that 
``the purpose of vision is very different when looking at a static scene to when engaging in real-world behavior.''  The interplay between  extracting visual information and coordinating the motor actions 
is a crucial issue to face for gaining an in-depth understanding of vision.  
One early realizes that manipulation of objects is not something
that we learn from a picture; it looks like you definitely need to act yourself if you want to 
gain such a skill. Likewise, the perception of the objects you manipulate 
can nicely get a reinforcement form such a mechanical feedback.
The mentioned interplay between perception and action finds an
intriguing convergence in the natural processes of gaze control and, overall, on 
the focus of attention~(\cite{DBLP:journals/ai/Ballard91}).
It looks like  {\em animate vision} goes beyond passive information extraction
and plays an important role in better posing most vision tasks.

%
% predictive coding
%
The studies in computer vision might benefit significantly also from the exploration of
the links with predictive coding~\cite{rao:natneuro99} that have had a remarkable impact in neuroscience.
In that framework one is willing to study theories of brain in which it constantly generates and updates a ``mental model''
of the environment. Overall, the model is supposed  to generate its own predictions of sensory input and 
compare them to the actual sensory input. The prediction error is expected to be used to update and revise the mental model.
While most of the studies in deep learning have been focused on the direct learning of object categories, 
there are a few contributions also in the direction of performing a sort of predictive coding by 
means of auto-encoding architectures~(\cite{DBLP:journals/corr/RonnebergerFB15}).
This neural network, which is referred to as an {\em U-net}, is used for medical image segmentation. 


\section{Dealing with video instead of images}
While the emphasis on methods rooted on still images is common on  most of nowadays 
state of the art object recognition approaches, in this paper we argue
 that there are strong arguments to start exploring the more natural visual interaction 
 that animals experiment in their own environment. 
The idea of shifting to video is very much 
related to the growing interest of {\em learning in the wild} that has been explored in the
last few years\footnote{See. e.g.~\url{https://sites.google.com/site/wildml2017icml/}.}.
The learning processes that take place in this kind of environments have a different
nature with respect to those that are typically considered in machine learning. 
%Learning convolutional nets on ImageNet typically consists of updating the weights
%from the processing of temporally unrelated images, whereas a video carries out
%information that is characterized by a smooth changes from close frames. 
While ImageNet~(\cite{imagenet_cvpr09}) is a collection of unrelated images, a video supports information only when motion is involved. In presence of still images that last for awhile, the
 corresponding stream of equal frames only conveys the information of a single image
 - apart from the duration of the interval in which the video has been kept constant. 
As a consequence,  visual environments mostly diffuse information only when
motion is involved. As time goes by, the information is only carried out by motion,
which modifies one frame to the next one according to the optical flow. Once we 
deeply capture this fundamental feature of vision,
we realize that a different theory of machine learning is needed that must be 
capable of naturally processing streams instead of a collection of independent images.   

%%\marginnote{Learning as the minimization of the cognitive action.}
%In this paper, the importance of motion invariance is stressed and, moreover,
%the solution is derived in the framework of the principle of 
%cognitive action~\cite{DBLP:journals/tcs/BettiG16}, which gives rise  to a
%time-variant differential equation, where the Lagrangian coordinates
%corresponds with the values of the convolutional filters. 
%It is pointed out that, under causality conditions, the well-position
%of the problems arises thanks to the process of video-blurring taking
%place at the beginning of learning, which has also been experimented
%in children. 
%The learning process can be interpreted in the framework of the minimization
%of the cognitive action that offers a self-consistent framework. In particular, if the video signal is almost periodic~\cite{besicovitch1954almost},
%then the computational model reduces to an asymptotically stable 
%differential equation that yields a sort of statistical consistency. 
%In this paper we mostly deal with a discussion of the principles that
%one should follow to construct a sound theory of vision that, later on, can 
%likely be also applied to computer vision. In addition, we discuss some of the
%reasons of the limitations of current approaches, where perceptual and linguistic
%tasks interwound with vision are not properly covered. This issue is enlighten 
%by proposing a hierarchy of cognitive tasks connected with vision that contributes
%to shed light on the intriguing connection between gaining perceptual and linguistic
%skills.  The discussion suggests that 

% eye movements and citation to nips
%\section{Cutting the umbilical cord with pattern recognition}
The scientific communities of pattern recognition and computer vision
have a longstanding tradition of strong intersections. 
As the notion of pattern began to circulate at the end of the 
Fifties, the discipline of pattern recognition grew up quickly
around the notion of pattern. No matter what kind of representation a
pattern is given, its name  conveys the  underlining assumption that,
regardless of the way they are obtained,
the recognition process involves single patterns. 
It is in fact their accumulation in appropriate collections which 
gives rise to statistical machine learning. 
While computer vision can hardly be delimited in terms both  of
methodologies and applications, the dominant foundations are
still the same promoted by the pioneers of pattern recognition.  
Surprisingly enough, there is no much attention on the crucial
role of the position (pixel) on which the decision is carried out
and, even more, the role of time in the recognition processes
doesn't seem to play a central role. 
It looks like we are mostly ignoring  that we are in front of
spatiotemporal information, whose reduction to isolated patterns
might not be a natural solution especially for the complex tasks
that we have been recently tackling. 

%\section{The long-standing tradition of pattern recognition}

%\subsection{The segmentation-recognition chicken-egg  dilemma}
In the last decades, the massive production of electronic documents,
along with their printed version, 
has given rise to specialized software tools to extract textual information
from optical data. Most optical documents, like 
tax forms or invoices, are characterized by a certain layout which
dramatically simplifies the process of information extraction. 
Basically, as one recognizes the class of a document, its layout
offers a significant prior on what we can expect to find in its
different areas. For those documents, the segmentation process 
can often be given a somewhat formal description, so as most of the problems are
reduced to deal with the presence of noise. As a matter of 
fact, in most real-world problems, the noise doesn't compromise
significantly the presence of segmentation, that is very well driven
by the expectations provided in each pixel of the documents.
These guidelines have been fueling the field of documental analysis
and recognition (DAR), whose growth in the last few years has led to
impressive results~(\cite{DBLP:journals/pami/MarinaiGS05}). 
Unfortunately, in most real-world problems, as we move to natural images and vision,
the methodology used in DAR is not really effective in most challenging problems.
The reason is that there is no longer a reliable anchor
to which one can cling for segmenting the objects 
of a scene. While we can provide a clear description of chars and 
lines in optical documents, the same doesn't hold for the picture
of a car which is mostly hidden by a truck during the overtaking. 
Humans exhibit a spectacular detection ability 
by simply relying on  small glimpses at different scale and 
rotations. In no way those a cognitive processes are reducible to
the well-posed segmentation problems of chars and lines in optical documents.
As we realize that there is a car, we can in fact provide its segmentation.
Likewise, if an oracle gives us the segmented portion of a car,
we can easily classify it. Interestingly, we don't really know 
which of the two processes is given a priority - if any. 
We are trapped into the chicken-egg dilemma on whether 
classification of objects must take place first of segmentation or vice versa.
Amongst others, this issue has been massively investigated by
in~(\cite{DBLP:conf/eccv/BorensteinU02})
and early pointed out in~(\cite{UllmanShimon1979Tiov}).
This intriguing dilemma might be connected with the 
absence of  focus of attention,
which necessarily leads to holistic mechanisms of information extraction.
Unfortunately, while holistic mechanisms are required at a certain level of abstraction, 
the segmentation is a truly local process that involves
low level features.
%Basically, there is no decoupling between the visual source and its linguistic description.  

The bottom line is that most problems
of computer vision are are posed according to the historical evolution of
the applications more than on an in-depth analysis of the underlying computational
processes. While this choice has been proven to be successful in many real-world
cases, stressing this research guideline might led, on the long run, 
to sterile directions. 
%%%%%%%%%%%%%%%
% invariances in the literature
%%%%%%%%%%%%%%%
Somewhat outside the mainstream of massive exploration of supervised 
learning, Poggio and Anselmi~(\cite{Poggio:2016:VCD}) pointed out the 
crucial role of incorporating appropriate visual invariances
into deep nets to go beyond the simple translation invariance 
that is currently characterizing convolutional networks. They propose an elegant mathematical framework 
on visual invariance and enlighten some intriguing neurobiological connections. 
Couldn't it be the case that the development of appropriate invariances is exactly what 
we need to go one step beyond?




==> bk/Introduction_4.tex <==
%%%% Prologue %%%%
%\subsection{Prologue}
The professional construction of huge supervised visual 
data bases has significantly contributed to the spectacular 
performance of deep learning. However, the extreme exploitation 
of the truly artificial communication protocol of supervised learning 
has been experimenting its drawbacks, including the vulnerability
to adversarial attacks, which might also be tightly connected to the
negligible role typically played by  the temporal structure.
Aren't we missing something?  It looks like Nature did a great job by using time to ``sew all the video frames'', whereas it  goes unnoticed to our eyes!  
At the dawn of pattern recognition, when we also began to cultivate the
idea of interpreting natural video, in order to simplify the problem 
of dealing with a huge amount of information we removed time, the connecting thread between frames, and began playing with 
the pattern regularities that emerge at the spatial level. As a consequence, all
tasks of pattern recognition were turned into problems
formulated on  collections of images, where 
the crucial role of temporal coherence was neglected. 
Interestingly, when considering the general problem of object recognition
and scene interpretation, the joint role of the computational resources and the access to huge visual databases of supervised data has 
contributed to erect nowadays
``reign of computer vision''.  
At a first glance this is reasonable, especially if you consider that video were
traditionally heavy data sources  to be played with. 
However, a closer look reveals that 
we are in fact neglecting a fundamental clue to interpret visual information, 
and that we have ended up into problems where the extraction of the visual concepts is mostly based on  spatial  regularities.
On the other hand, reigns have typically consolidated rules from which it's hard to escape.  This is common in novels and real life.
``The Three Princes of Serendip'' is the English version of ``Peregrinaggio di tre giovani figliuoli del re di Serendippo,'' published by Michele Tramezzino in Venice on 1557. These princes journeyed widely, and as they traveled they continually made discoveries, by accident and sagacity, of things they were not seeking. A couple of centuries later, in a letter of January 28, 1754 to a British envoy in Florence, the English politician and writer Horace Walpole coined a new term: serendipity, which is succinctly characterized as the art of finding something when searching for something else. Couldn't similar travels open new
scenario in computer vision? Couldn't the visit to 
well-established scientific domains, where time is dominating the scene, 
open new doors to an in-depth understanding of vision? 
We need to stitch the frames to recompose the video using time as a thread, the same thread we had extracted to work on the images at the birth of the discipline.
We need to go beyond a peaceful interlude and think of 
learning theories based on video more than on images!
%%%%%%%

This paper is a travel towards the frontiers of the science of vision with special emphasis
to object perception. We drive the discussion by a number
of  curios questions that mostly arise
as one tries to interpret and disclose natural vision processes 
in a truly computational framework. Unfortunately, as yet, we are far away
from addressing the posed questions. However, this paper comes from the 
awareness that posing right questions on the discipline might themselves stimulate 
its progress. 


\section{Cutting the umbilical cord with pattern recognition}
\label{Unbilicalsec}
%%% Roli's comments 
In the eighties, Satosi Watanabe wrote a seminal book~(\cite{10.5555/4394}) 
in which he early pointed out the different facets of pattern recognition that
can be regarded as  perception, categorization,  induction, pattern recognition,
as well  as statistical decision making.
Most of the modern work on computer vision for object perception fits with 
Watanabe's view of pattern recognition as statistical decision making and pattern recognition as categorization.
%
Based on optimization schemes with billions of variables and universal  
approximation capabilities, the spectacular results of deep learning have elevated 
this view of pattern recognition to a position where it is hardly debatable. 
While the emphasis on a general theory of vision was already 
the main objective at the dawn of the discipline~(\cite{Marr82}), 
its evolution has been mostly marked to significant experimental achievements. 
Most successful approaches  seem to be the natural outcome of a very well-established tradition in pattern recognition methods working on images, which have given rise to nowadays emphasis on collecting big labelled image databases (e.g.~\cite{imagenet_cvpr09}).

%
% epistemological issue
%
However, in spite of these successful results, this could be the time of an in-depth rethinking of what we have 
been doing, especially by considering the remarkable traditions of the 
overall field of vision.  In his seminal book,
Freeman J. Dyson~(\cite{dyson2004infinite}),  discusses two distinct styles of scientific thinking: unifying and diversifying. He claimed that most sciences are dominated by one or the other in various periods of their history. Unifiers are people whose driving passion is to find general principles, whereas 
Diversifiers are people with the passion of details. 
Historical progress of science is often a blend of unification and diversification. 
Couldn't it be the right time to exploit the impressive literature in the field vision
to conquer a more unified view of object perception? 

%
% Cognitive Ethology
%

In the last few years, a number of studies in psychology cognitive science have 
been pushing truly novel
approaches to vision. In~(\cite{Kingstone2010}), it is pointed out that 
a critical problem that continues to bedevil the study of human cognition is related to 
the  remarkably successes gained in experimental psychology, where 
one is typically involved in simplifying
the experimental context  with the purpose to discover causal relationships. 
In so doing we minimize the complexity of the environment and maximize the experimental control,
which is typically done also in computer vision when we face object recognition. 
However, one might ask whether such a simplification is really adequate and, most
importantly, if it is indeed a simplification. Are we sure that treating vision as a collection
of unrelated frames leads to simplification of learning visual tasks? 
In this paper we argue this not the case, since 
cognitive processes vary substantially with changes in context. 
When promoting the actual environmental interaction,~\cite{Kingstone2010}
introduce a novel research approach, called, ``Cognitive Ethology'', 
where one opts to explore first how people behave in a truly naturally situation. 
Once we have collected experience and evidence in the actual environment then 
we can move into the laboratory to test hypotheses.  This strongly suggests
that also machines should learn in the wild!

%
% vision as action ... in addition to vision as perception
%

Other fundamental lessons come from the school of robotics
for whatever involves the control of object-directed actions. 
In~(\cite{Ballard2011}), it is pointed out that 
``the purpose of vision is very different when looking at a static scene to when engaging in real-world behavior.''  The interplay between  extracting visual information and coordinating the motor actions 
is a crucial issue to face for gaining an in-depth understanding of vision.  
One early realizes that manipulation of objects is not something
that we learn from a picture; it looks like you definitely need to act yourself if you want to 
gain such a skill. Likewise, the perception of the objects you manipulate 
can nicely get a reinforcement form such a mechanical feedback.
The mentioned interplay between perception and action finds an
intriguing convergence in the natural processes of gaze control and, overall, on 
the focus of attention~(\cite{DBLP:journals/ai/Ballard91}).
It looks like  {\em animate vision} goes beyond passive information extraction
and plays an important role in better posing most vision tasks.

%
% predictive coding
%
The studies in computer vision might benefit significantly also from the exploration of
the links with predictive coding~\cite{rao:natneuro99} that have had a remarkable impact in neuroscience.
In that framework one is willing to study theories of brain in which it constantly generates and updates a ``mental model''
of the environment. Overall, the model is supposed  to generate its own predictions of sensory input and 
compare them to the actual sensory input. The prediction error is expected to be used to update and revise the mental model.
While most of the studies in deep learning have been focused on the direct learning of object categories, 
there are a few contributions also in the direction of performing a sort of predictive coding by 
means of auto-encoding architectures~(\cite{DBLP:journals/corr/RonnebergerFB15}).
This neural network, which is referred to as an {\em U-net}, is used for medical image segmentation. 


\section{Dealing with video instead of images}
While the emphasis on methods rooted on still images is common on  most of nowadays 
state of the art object recognition approaches, in this paper we argue
 that there are strong arguments to start exploring the more natural visual interaction 
 that animals experiment in their own environment. 
The idea of shifting to video is very much 
related to the growing interest of {\em learning in the wild} that has been explored in the
last few years\footnote{See. e.g.~\url{https://sites.google.com/site/wildml2017icml/}.}.
The learning processes that take place in this kind of environments have a different
nature with respect to those that are typically considered in machine learning. 
%Learning convolutional nets on ImageNet typically consists of updating the weights
%from the processing of temporally unrelated images, whereas a video carries out
%information that is characterized by a smooth changes from close frames. 
While ImageNet~(\cite{imagenet_cvpr09}) is a collection of unrelated images, a video supports information only when motion is involved. In presence of still images that last for awhile, the
 corresponding stream of equal frames only conveys the information of a single image
 - apart from the duration of the interval in which the video has been kept constant. 
As a consequence,  visual environments mostly diffuse information only when
motion is involved. As time goes by, the information is only carried out by motion,
which modifies one frame to the next one according to the optical flow. Once we 
deeply capture this fundamental feature of vision,
we realize that a different theory of machine learning is needed that must be 
capable of naturally processing streams instead of a collection of independent images.   

%%\marginnote{Learning as the minimization of the cognitive action.}
%In this paper, the importance of motion invariance is stressed and, moreover,
%the solution is derived in the framework of the principle of 
%cognitive action~\cite{DBLP:journals/tcs/BettiG16}, which gives rise  to a
%time-variant differential equation, where the Lagrangian coordinates
%corresponds with the values of the convolutional filters. 
%It is pointed out that, under causality conditions, the well-position
%of the problems arises thanks to the process of video-blurring taking
%place at the beginning of learning, which has also been experimented
%in children. 
%The learning process can be interpreted in the framework of the minimization
%of the cognitive action that offers a self-consistent framework. In particular, if the video signal is almost periodic~\cite{besicovitch1954almost},
%then the computational model reduces to an asymptotically stable 
%differential equation that yields a sort of statistical consistency. 
%In this paper we mostly deal with a discussion of the principles that
%one should follow to construct a sound theory of vision that, later on, can 
%likely be also applied to computer vision. In addition, we discuss some of the
%reasons of the limitations of current approaches, where perceptual and linguistic
%tasks interwound with vision are not properly covered. This issue is enlighten 
%by proposing a hierarchy of cognitive tasks connected with vision that contributes
%to shed light on the intriguing connection between gaining perceptual and linguistic
%skills.  The discussion suggests that 

% eye movements and citation to nips
%\section{Cutting the umbilical cord with pattern recognition}
The scientific communities of pattern recognition and computer vision
have a longstanding tradition of strong intersections. 
As the notion of pattern began to circulate at the end of the 
Fifties, the discipline of pattern recognition grew up quickly
around the notion of pattern. No matter what kind of representation a
pattern is given, its name  conveys the  underlining assumption that,
regardless of the way they are obtained,
the recognition process involves single patterns. 
It is in fact their accumulation in appropriate collections which 
gives rise to statistical machine learning. 
While computer vision can hardly be delimited in terms both  of
methodologies and applications, the dominant foundations are
still the same promoted by the pioneers of pattern recognition.  
Surprisingly enough, there is no much attention on the crucial
role of the position (pixel) on which the decision is carried out
and, even more, the role of time in the recognition processes
doesn't seem to play a central role. 
It looks like we are mostly ignoring  that we are in front of
spatiotemporal information, whose reduction to isolated patterns
might not be a natural solution especially for the complex tasks
that we have been recently tackling. 

%\section{The long-standing tradition of pattern recognition}

%\subsection{The segmentation-recognition chicken-egg  dilemma}
In the last decades, the massive production of electronic documents,
along with their printed version, 
has given rise to specialized software tools to extract textual information
from optical data. Most optical documents, like 
tax forms or invoices, are characterized by a certain layout which
dramatically simplifies the process of information extraction. 
Basically, as one recognizes the class of a document, its layout
offers a significant prior on what we can expect to find in its
different areas. For those documents, the segmentation process 
can often be given a somewhat formal description, so as most of the problems are
reduced to deal with the presence of noise. As a matter of 
fact, in most real-world problems, the noise doesn't compromise
significantly the presence of segmentation, that is very well driven
by the expectations provided in each pixel of the documents.
These guidelines have been fueling the field of documental analysis
and recognition (DAR), whose growth in the last few years has led to
impressive results~(\cite{DBLP:journals/pami/MarinaiGS05}). 
Unfortunately, in most real-world problems, as we move to natural images and vision,
the methodology used in DAR is not really effective in most challenging problems.
The reason is that there is no longer a reliable anchor
to which one can cling for segmenting the objects 
of a scene. While we can provide a clear description of chars and 
lines in optical documents, the same doesn't hold for the picture
of a car which is mostly hidden by a truck during the overtaking. 
Humans exhibit a spectacular detection ability 
by simply relying on  small glimpses at different scale and 
rotations. In no way those a cognitive processes are reducible to
the well-posed segmentation problems of chars and lines in optical documents.
As we realize that there is a car, we can in fact provide its segmentation.
Likewise, if an oracle gives us the segmented portion of a car,
we can easily classify it. Interestingly, we don't really know 
which of the two processes is given a priority - if any. 
We are trapped into the chicken-egg dilemma on whether 
classification of objects must take place first of segmentation or vice versa.
Amongst others, this issue has been massively investigated by
in~(\cite{DBLP:conf/eccv/BorensteinU02})
and early pointed out in~(\cite{UllmanShimon1979Tiov}).
This intriguing dilemma might be connected with the 
absence of  focus of attention,
which necessarily leads to holistic mechanisms of information extraction.
Unfortunately, while holistic mechanisms are required at a certain level of abstraction, 
the segmentation is a truly local process that involves
low level features.
%Basically, there is no decoupling between the visual source and its linguistic description.  

The bottom line is that most problems
of computer vision are are posed according to the historical evolution of
the applications more than on an in-depth analysis of the underlying computational
processes. While this choice has been proven to be successful in many real-world
cases, stressing this research guideline might led, on the long run, 
to sterile directions. 
%%%%%%%%%%%%%%%
% invariances in the literature
%%%%%%%%%%%%%%%
Somewhat outside the mainstream of massive exploration of supervised 
learning, Poggio and Anselmi~(\cite{Poggio:2016:VCD}) pointed out the 
crucial role of incorporating appropriate visual invariances
into deep nets to go beyond the simple translation invariance 
that is currently characterizing convolutional networks. They propose an elegant mathematical framework 
on visual invariance and enlighten some intriguing neurobiological connections. 
Couldn't it be the case that the development of appropriate invariances is exactly what 
we need to go one step beyond?




==> bk/ST.tex <==
\section{Computational models in spatiotemporal environments}

%
% Q2, Q3, Q4
%

The extraction of informative and robust cues from visual scenes
has been attracting more and more interest in computer vision. 
For many years, scientists and engineers have contributed to the construction
of solutions to extract visual features, that are mostly based on  clever heuristics
(see e.g.~\cite{sift2004}). However, the remarkable achievements  of the last 
few years have been mostly based on the accumulation of huge visual collections 
enriched by crowdsourcing. It has created labels to carry out massive supervised learning 
in deep convolutional networks, that has given rise to very effective 
internal representations of visual features. The  have been successfully used
in an impressive number of application (see e.g.
~\cite{NIPS2012_4824},\cite{DBLP:journals/corr/SimonyanZ14a}).

In this book, we argue that while stressing this issue we 
have been facing artificial problems that, from a pure computational point of view, 
are likely to be significantly more complex than natural visual tasks 
that are daily faced by animals. In humans, the emergence of cognition from visual
environments is interwound with language. This often leads to attack
the interplay between visual and linguistic skills by simple models
that, like for supervised learning, strongly rely on linguistic attachment.
However, when observing the spectacular skills of the eagle that catches the pray,
one promptly realizes that for an in-depth understanding
of vision, that likely yields also an impact in computer implementation,
one should begin with a neat separation with language! 
This paper is mostly motivated by the curiosity of addressing a number
of questions that arise when looking at natural visual processes~\cite{Betti2018-CN-arxiv}.
While they come from natural observation, they are mostly regarded
as general issues strongly rooted in information-based principles, that we
conjecture are of primary importance also in computer vision.

%A good theory on object recognition proposed needs a computational perspective of
%vision regardless of the ``body'' which sustains the processing. 
%In particular, the theory addresses some fundamental questions, reported below,
%that involve vision processes taking place in both animals and machines. 
\section{Animals and computers}
discuss from Boccignone's references to chicks' experiments. What about
one-shot learning? Clearly it's a matter of a sort of transfer learning which 
takes place at the birth of animals. The genetics plays a fundamental role
in defining basic architectural structures by its encoding, but most of the
actual architecture for vision is developed while learning in the
environment. It's worth mentioning that the only information that you can actually
transfer at the time of conception is encoded in the fetus. Sexual reproduction
assumes that  ...
humane genome and the amount of info which is encoded for any 
human action. A lot of other additional information is for learning!
In vision is the same ... you must encode info which facilitates the 
task of object recognition and, at the same time, the task of object avoidance. 
In one case we need motion invariance, whereas in the other case you need
maximal reaction to motion.


 
\section{Are we missing something?}
\section{Scholia}



==> bk/Umbilical.tex <==
The scientific communities of pattern recognition and computer vision
have a longstanding tradition with strong intersections. 
As the notion of pattern began to circulate at the end of the 
Fifties, the discipline of pattern recognition grew up quickly
around that notion. No matter what kind of representation a
pattern is given, its name  conveys the  underlining assumption that,
regardless of the way they are obtained,
the recognition process involves single patterns. 
It is in fact their accumulation in appropriate collections which 
gives rise to statistical machine learning. 

While computer vision can hardly be delimited both in terms of
methodologies and applications, the dominant foundations are
still the same promoted by the pioneers of pattern recognition.  
Surprisingly enough, there is no much attention on the crucial
role of the position (pixel) on which the decision is carried out
and, even more, the role of time in the recognition processes
doesn't seem to play a central role. 
It looks like we are mostly ignoring  that we are in front of
spatiotemporal information, whose reduction to isolated patterns
might not be natural solution especially for the complex tasks
that we have been recently tackling. 

%\section{The long-standing tradition of pattern recognition}

\section{The segmentation-recognition chicken-egg  dilemma}
In the last decades, the massive production of electronic documents,
along with their printed version, 
has given rise to specialized software tools to extract textual information
from optical representations. Most optical documents, like 
tax forms or invoices, are characterized by a certain layout which
dramatically simplifies the process of information extraction. 
Basically, as one recognizes the class of document, its layout
offers a significant prior on what we can expect to find in its
different areas. For these documents, the segmentation process 
can be given a formal description, so as most of the problems are
reduced to deal with the presence of noise. As a matter of 
fact, in most real-world problems, the noise doesn't compromise
significantly the presence of segmentation, that is very well driven
by the expectations provided in each pixel of the documents.
This guidelines have been fueling the field of documental analysis
and recognition (DAR), whose growth in the last few years has led to
impressive results.
Unfortunately, as we move to natural images and vision,
the methodology used in DAR, in most real-world problems, leads
to controversial results. The reason is that there is no reliable 
anchor anymore  to which one can hang for segmenting the objects 
of a scene. While we can provide a clear description of chars and 
lines in optical documents, the same doesn't hold for the picture
of a car which is mostly hidden by a truck during the overtaking. 
Humans exhibit a spectacular ability of detecting the car also 
by simply relying on a very small portion at different scale and 
rotations. In no way such a cognitive process is reducible to
the well-posed segmentation of chars and lines in optical documents.
As we realize that there is a car, we can in fact provide its segmentation.
Likewise, if an oracle gives us the segmented portion of the car
we can easily classify it. Interestingly, we don't really know 
which of the two processes is given a priority - if any. 
We are trapped into the chicken-egg dilemma on whether 
classification of objects or segmentation must take place first. 
This is due to the absence of any focus of attention,
which necessarily leads to holistic mechanisms of information extraction.
Unfortunately, while holistic mechanisms are required at a certain level of abstraction, the segmentation is a truly local process that involves
low level features.
%Basically, there is no decoupling between the visual source and its linguistic description.  


\section{Beyond the links with pattern recognition}
% v(x,t) instead of z^d
A good theory of vision seems to require a direct treatment of
the video signal $v(x,t)$ more that properly segmented patterns
to be used for feeding machine learning based classifiers.
Decisions at pixel level at any time are expected to be 
achieved by a visual agent. Clearly, this poses the question 
on the meaning of performing spatiotemporal local decisions 
at $(x,t)$, as well their connection with more abstract cognitive
processes that allow humans to provide symbolic descriptions
of objects and scenes. The umbilical cut with pattern recognition
is required to spread the idea that one must not necessarily
need to segment the visual scene in 


% local vs global decisions 

\section{Focus of attention}

\section{Scholia}

==> bk/Umbilical_2.tex <==
The scientific communities of pattern recognition and computer vision
have a longstanding tradition with strong intersections. 
As the notion of pattern began to circulate at the end of the 
Fifties, the discipline of pattern recognition grew up quickly
around the notion of pattern. No matter what kind of representation a
pattern is given, its name  conveys the  underlining assumption that,
regardless of the way they are obtained,
the recognition process involves single patterns. 
It is in fact their accumulation in appropriate collections which 
gives rise to statistical machine learning. 

While computer vision can hardly be delimited in terms both  of
methodologies and applications, the dominant foundations are
still the same promoted by the pioneers of pattern recognition.  
Surprisingly enough, there is no much attention on the crucial
role of the position (pixel) on which the decision is carried out
and, even more, the role of time in the recognition processes
doesn't seem to play a central role. 
It looks like we are mostly ignoring  that we are in front of
spatiotemporal information, whose reduction to isolated patterns
might not be a natural solution especially for the complex tasks
that we have been recently tackling. 

%\section{The long-standing tradition of pattern recognition}

\subsection{The segmentation-recognition chicken-egg  dilemma}
In the last decades, the massive production of electronic documents,
along with their printed version, 
has given rise to specialized software tools to extract textual information
from optical data. Most optical documents, like 
tax forms or invoices, are characterized by a certain layout which
dramatically simplifies the process of information extraction. 
Basically, as one recognizes the class of a document, its layout
offers a significant prior on what we can expect to find in its
different areas. For these documents, the segmentation process 
can often be given a somewhat formal description, so as most of the problems are
reduced to deal with the presence of noise. As a matter of 
fact, in most real-world problems, the noise doesn't compromise
significantly the presence of segmentation, that is very well driven
by the expectations provided in each pixel of the documents.
These guidelines have been fueling the field of documental analysis
and recognition (DAR), whose growth in the last few years has led to
impressive results.
Unfortunately, as we move to natural images and vision,
the methodology used in DAR, in most real-world problems, leads
to controversial results. The reason is that there is no longer a reliable anchor
to which one can cling for segmenting the objects 
of a scene. While we can provide a clear description of chars and 
lines in optical documents, the same doesn't hold for the picture
of a car which is mostly hidden by a truck during the overtaking. 
Humans exhibit a spectacular ability of detecting the car also 
by simply relying on a very small portion at different scale and 
rotations. In no way such a cognitive process is reducible to
the well-posed segmentation of chars and lines in optical documents.
As we realize that there is a car, we can in fact provide its segmentation.
Likewise, if an oracle gives us the segmented portion of the car
we can easily classify it. Interestingly, we don't really know 
which of the two processes is given a priority - if any. 
We are trapped into the chicken-egg dilemma on whether 
classification of objects must take place first of segmentation or vice versa.
This is due to the absence of any focus of attention,
which necessarily leads to holistic mechanisms of information extraction.
Unfortunately, while holistic mechanisms are required at a certain level of abstraction, 
the segmentation is a truly local process that involves
low level features.
%Basically, there is no decoupling between the visual source and its linguistic description.  


\subsection{Beyond the links with pattern recognition}
% v(x,t) instead of z^d
A good theory of vision seems to require a direct treatment of
the video signal $v(x,t)$ more that properly segmented patterns
to be used for feeding machine learning based classifiers.
Decisions at pixel level at any time are expected to be 
achieved by a visual agent. Clearly, this poses the question 
on the meaning of performing spatiotemporal local decisions 
at $(x,t)$, as well their connection with more abstract cognitive
processes that allow humans to provide symbolic descriptions
of objects and scenes. The umbilical cut with pattern recognition
is required to spread the idea that one must not necessarily
need to segment the visual scene in 


% local vs global decisions 

\subsection{En plain air}

\subsection{Ten questions}




==> bk/Umbilical_3.tex <==
The scientific communities of pattern recognition and computer vision
have a longstanding tradition with strong intersections. 
As the notion of pattern began to circulate at the end of the 
Fifties, the discipline of pattern recognition grew up quickly
around the notion of pattern. No matter what kind of representation a
pattern is given, its name  conveys the  underlining assumption that,
regardless of the way they are obtained,
the recognition process involves single patterns. 
It is in fact their accumulation in appropriate collections which 
gives rise to statistical machine learning. 

While computer vision can hardly be delimited in terms both  of
methodologies and applications, the dominant foundations are
still the same promoted by the pioneers of pattern recognition.  
Surprisingly enough, there is no much attention on the crucial
role of the position (pixel) on which the decision is carried out
and, even more, the role of time in the recognition processes
doesn't seem to play a central role. 
It looks like we are mostly ignoring  that we are in front of
spatiotemporal information, whose reduction to isolated patterns
might not be a natural solution especially for the complex tasks
that we have been recently tackling. 

%\section{The long-standing tradition of pattern recognition}

\subsection{The segmentation-recognition chicken-egg  dilemma}
In the last decades, the massive production of electronic documents,
along with their printed version, 
has given rise to specialized software tools to extract textual information
from optical data. Most optical documents, like 
tax forms or invoices, are characterized by a certain layout which
dramatically simplifies the process of information extraction. 
Basically, as one recognizes the class of a document, its layout
offers a significant prior on what we can expect to find in its
different areas. For these documents, the segmentation process 
can often be given a somewhat formal description, so as most of the problems are
reduced to deal with the presence of noise. As a matter of 
fact, in most real-world problems, the noise doesn't compromise
significantly the presence of segmentation, that is very well driven
by the expectations provided in each pixel of the documents.
These guidelines have been fueling the field of documental analysis
and recognition (DAR), whose growth in the last few years has led to
impressive results.
Unfortunately, as we move to natural images and vision,
the methodology used in DAR, in most real-world problems, leads
to controversial results. The reason is that there is no longer a reliable anchor
to which one can cling for segmenting the objects 
of a scene. While we can provide a clear description of chars and 
lines in optical documents, the same doesn't hold for the picture
of a car which is mostly hidden by a truck during the overtaking. 
Humans exhibit a spectacular ability of detecting the car also 
by simply relying on a very small portion at different scale and 
rotations. In no way such a cognitive process is reducible to
the well-posed segmentation of chars and lines in optical documents.
As we realize that there is a car, we can in fact provide its segmentation.
Likewise, if an oracle gives us the segmented portion of the car
we can easily classify it. Interestingly, we don't really know 
which of the two processes is given a priority - if any. 
We are trapped into the chicken-egg dilemma on whether 
classification of objects must take place first of segmentation or vice versa.
This is due to the absence of any focus of attention,
which necessarily leads to holistic mechanisms of information extraction.
Unfortunately, while holistic mechanisms are required at a certain level of abstraction, 
the segmentation is a truly local process that involves
low level features.
%Basically, there is no decoupling between the visual source and its linguistic description.  


\subsection{Beyond the links with pattern recognition}
% v(x,t) instead of z^d
A good theory of vision seems to require a direct treatment of
the video signal $v(x,t)$ more that properly segmented patterns
to be used for feeding machine learning based classifiers.
Decisions at pixel level at any time are expected to be 
achieved by a visual agent. Clearly, this poses the question 
on the meaning of performing spatiotemporal local decisions 
at $(x,t)$, as well their connection with more abstract cognitive
processes that allow humans to provide symbolic descriptions
of objects and scenes. The umbilical cut with pattern recognition
is required to spread the idea that one must not necessarily
need to segment the visual scene in 


% local vs global decisions 

\subsection{En plain air}

\subsection{Ten questions}




==> bk/a.tex <==
%
% object identity vs abstract objection notion
%
\section{Visual skills and abstraction}
% object identity
Human visual skills are somewhat astonishing. We get in touch with the spectacular capabilities of
interpreting visual scene whenever we open the challenge of describing the underlying computational process.
\marginpar{\small Object identity}
From one side, humans we can recognize the objects identity regardless of the different poses in which they come. 
This is quite surprising! Objects are available in different positions, at different scales and rotations, 
they can be deformable and obstructed. Only small portions can be enough for their detection, even in 
presence of environmental noise. Children recognize their Teddy Bear from different angles. As
they bite it, not only does the Bear deform as a result, but they experience a very peculiar sight of it. Yet,
they perceive it consistently. Deep learning has been proven to be very effective to replicate those
visual capabilities provided that we rely on tons of supervisions. 
However, you can't really hope to recognize your bear, if the only thing that distinguishes it from another is that 
it is slightly torn behind the head. It is that torn part that gives it its identity. 
Therefore, when dealing with some real contexts, the supervised learning approach cannot really 
aspire to reach the human capacity to define the identity of objects.

\marginpar{\small Object affordance}
% object abstraction
Humans, and likely most animals, also conquer a truly different understanding of visual scene that
goes beyond the conceptualization with single object identities.
In early Sixties, James J. Gibson coined the {\em affordance} in~\cite{Gibson1966}, even though 
a more refined analysis came later in~\cite{plasticq}. In his own words:
\begin{quote}{\em
The affordances of the environment are what it {\em offers} the animal, what it {\em provides} 
or furnishes, either for good or ill. The verb to {\em afford} is found in the dictionary, the noun affordance is not. I have made it up. I mean by it something that refers to both the environment and the animal in a way that no existing term does. It implies the complementarity of the animal and the environment.
}\end{quote}
Affordance makes sense for a species of animal, where specific actions take place.
A chair, for example, has the affordance of seating a human being, but can have 
many other potential uses. We can climb on it to reach a certain object or we 
can use it to defend ourselves from someone armed with a knife.
inadequacy.  It was also early clear that no all objects convey significant information
from their affordance. In~\cite{plasticq}, the distinction between {\em attached and detached objects}
clearly indicates that  some can neither be moved nor easily broken. While our home can be given
an affordance, it is attached to the earth and cannot be grasped. Interestingly, while a small cube is 
graspable, huge cubes are not. However, a huge cube can still be graspable by an appropriate ``handle.'' 
Basically,  one can think of object perception in terms of its properties and qualities. 
However, this is strictly connected to the object identity, whereas most common and useful way of 
gaining the notion of objects likely comes from their affordances. 
The object affordance is what humans -- and animals -- normally pay attention to. 
As  infants begin their environmental experiences they likely look at object meaning more
then at the surface, at the color or at form. This interpretation is kept during our ordinary 
environmental interactions. 
\marginpar{\small Do we really need to classify objects?}
The notion of object  affordance  somewhat challenges the apparently indisputable philosophical 
muddle of assuming fixed classes of objects. This is a slippery issue! To what extent can we 
regard object recognition as a classification problem? Clearly, 
there is no need to classify objects in order to understand what they are for. 
Hence, we could considering the advantages of of moving from nowadays dominating computer vision  
approach to a truly ecological viewpoint that suggest experimenting niches based set of well-defined, typically
limited object affordances.


\section{Objection affordance by motion invariance}
Seminal Gibson's contributions~\cite{Gibson1966,plasticq} have inspired scientists for decades. 
His studies in the field of psychology have been contaminating the community of computer vision
(see e.g.~\cite{DBLP:conf/cvpr/GallFG11}) also in the era of deep learning~\cite{hassanin2018visual}.
However, it looks like the in-depth studies that gave rise to the notion of affordance haven't been found 
an appropriate translation into a computational model yet. Object affordance is interwound with correspondent
actions, but studies on these topics are mostly carried out independently one of each other in computer vision. 
Interestingly, the interpretation of actions is typically regarded as sequential process. Aren't actions the 
outcome of a sequence of frames? Studies in deep learning somehow aggregate features and optical flow,
but sequences are always taken into account mostly by combining Convolutional Neural Networks
and Long-Short-Term Memory recurrent neural networks~\cite{DBLP:journals/sensors/ZhangZZLYDC19}. 
\marginpar{\small Picture perceivable actions}
However, humans can promptly perceive many common actions and object affordance from single pictures!
For example, we can easily recognize the act of jumping, as well as the act of pouring a liquid into a container.
 Hence, it looks like there are actions that are perceived from single
pictures without presenting video clips. How can this be possible? Before addressing this question, 
it's important to realize that when shifting attention to actions, we need to pay attention to their in-depth
meaning that is especially paired with sophisticated human experiences.
While we can recognize from a single picture the act of pouring a liquid into a container, which nicely yields  the correspondent
affordance, we cannot recognize the act of solving Rubik's cube. A single picture can only yields suspiciousness
on the acts of killing but cannot guarantee to drive the conclusion. Similarly, a photo in which I'm trying to make myself the bow
doesn't not really correspond with the action labelled as ``how to tie the perfect bow'', since the photo could just 
trace my beginning act which might not result in a successful tie of the perfect bow! 
The acts of solving the Rubik's cube, killing, and tying the bow do require video clips for their interpretation, whereas 
other actions, like running, jumping, grazing the grass, and pouring a liquid into a container are {\em picture perceivable}.
The natural flow of time conveys a sort of direction to actions like seating and standing up; they are similar, 
yet somewhat opposite in their meaning. The same holds for the act of killing and cutting the bread. 
We can hit with the knife or remove it from an injured person. Clearly, the simple act of removal can support an
important difference: the person who's acting might be the killer, who's just removing the knife for hitting again, or 
might be a policeman who has just been notified of the murder. Those actions definitely need 
a sequence-based analysis for their interpretation and they also support a different affordance. 
however, they refer to the same object (e.g. the chair and the knife), which means that the process of object 
recognition generally involves multiple affordances. The notion of chair clearly arises from the acts of seating and standing up.

\marginpar{Object pairing $p \bowtie o$ and optical flow} 
Like for object identification, the notion on affordance becomes more clear when  shifting
attention at pixel level, which is what foveate animals do. First, we need to assume a sort of animal-centric view 
since object affordance can only be driven by an animal. Without limitation of generalities, suppose we are
dealing with human actions, and let us consider a pixel $x$ where both a person, with object identity $p(x,t)$, 
and an object, with identity  $o(x,t)$, are both detected. In general you can also assume that the object
defined by $o(x,t)$ is not necessarily referring to a person, but to tools typically used in human actions.
For instance, $o(x,t)$ could be the identifier of a 
hammer which is used to hang a picture. Interestingly, a pixel could contain the identity of the hammer, the picture
and the fingers of a person. In general, it could be the case that more than one 
object are defined at $(x,t)$ which depends on the extent to which we consider the contextual information.  
In that case we may have more than one optical flow at $(x,t)$. However, for the sake of simplicity, suppose
the optical flow defined by $v(x,t)$ in pixel $x$ at time $t$ comes from the person who's providing the
object affordance. In this case, in addition to the identification code  $o(x,t)$, the person $p(x,t)$
provides the object affordance $\alpha_{p}(x,t)$  that is associated with the action $a_{p}(x,t)$ carried out
by $p(x,t)$. Notice that while the computation of the affordance is based on visual features, the action
also includes the optical flow which, as already stated, can be interpreted as a feature itself. 
The object $o(x,t)$ could also be subjected to motion that contribute to the interpretation of the associated action.
Now let $P(t) \subset R$ and $O(t) \subset R$ be 
the segments of the retina $R$ that characterize the objects with codes $p$ and $o$, respectively. Furthermore, let 
$V_{p}(t),V_{o}(t) \subset R$ the subsets of the retina with non-vanishing optical flow produced by the 
person $p(x,t)$ and the object $o(x,t)$, respectively. More precisely, we assume that we are focusing
attention at $f(x,t)$ and that  $V_{p}(t),V_{o}(t)$ are the graphs generated by the non-vanishing optical flows
and that, in general, all the pixels involved in $V(t)=V_{p}(t) \cup V_{o}(t)$ are useful. 
We can define the affordance for 
object identified by $o(x,t)$ by considering $A_{p \bowtie o}(t) = P(t) \cap O(t) \cap V(t)$.  
During the agent's life over the horizon $T \subset \bbR$
the object $o$ and the person $p$ define the object affordance  by 
$A_{p \bowtie o} = \{A_{o}(t), \forall t \in T \}$. Moreover, during the agent's life,  all the object identifiers $I_{1}$ 
turn out to be associated with $I_{2}$ which also perform actions, thus defining the affordance relation
$\mathscr{A} \subset I_{1} \times I_{2}:=\{(p,o) \in  I_{1} \times I_{2}: \ \ p \bowtie o\}$.
\marginpar{\small Gaining object affordance by motion invariance}
We can formulate the problem of learning by imposing
the pairwise invariance that arises from the pairing $p \bowtie o$ for both the action and the correspondent affordance as follows:
 \begin{equation}
 	  \forall (p,o) \in \mathscr{A}, \ \forall (x,t) \in A_{p \bowtie o} \ \   
	  [\nabla_{(x,t)} a_{p}(x,t)=0]\land [\nabla_{(x,t)} \alpha_{p}(x,t)=0].
\label{AffordanceMO}
 \end{equation}
This constraint compactly states that whenever $o$ meets the moving object $p$ they join by $\bowtie$
so as $p$ propagate affordance information to $o$ with the purpose of constructing $\alpha$.
The identifiers $p$ and $o$ turn out to be joined thanks to the action, defined by $a$, that is carried out by $p$.
The affordance propagation arises from the spatiotemporal invariance that is imposed by operator $\nabla_{(x,t)}$.
Basically, during the agent's life $p$ and $o$ are joined over $A_{p \bowtie o}$ and one wants to 
impose the affordance the same affordance $\alpha_{p}$ that emerges from the same action $a_{p}$.
It's worth mentioning that the same person $p$ can propagate the same affordance $\alpha_{p}$
to objects with different object identity $o_{1},o_{2}$. This generates a partition on the set $O$ of 
object identifiers by the relation
\begin{equation}
	o_{1} \stackrel{p}{\sim} o_{2} \leftrightarrow (p \bowtie o_{1}) \land  (p \bowtie o_{2}).
\end{equation}
Interestingly, two persons, defined by $p_{1},p_{2}$ can also yield the same affordance on $o$,
which is represented by the dual condition
\begin{equation}
	p_{1} \stackrel{o}{\sim} p_{2} \leftrightarrow (p_{1} \bowtie o) \land  (p_{2} \bowtie o).
\end{equation}
The maximum degree of abstraction is gained when the propagated affordance 
is independent of the person. In this case  $p_{1} \stackrel{o}{\sim} p_{2}$
is true regardless of the pair $p_1,p_2$ and $o_{1} \stackrel{p}{\sim} o_{2}$
can simply be replaced with $o_{1} \sim o_{2}$. In this special case the partition on $O$
simply yields the quotient space ${\cal Q}=O / \sim$ where the equivalent classes can be thought of 
the class of the object.

\marginpar{\small Do we really need to know the object identifiers to generate the affordances?}
It's worth mentioning that in the above discussion we involved the object identifiers, so 
that one can legitimately ask whether the affordance can be gained also by ignoring the object identity. 
Notice that while the object identity is gained by motion invariance of the same object, 
its affordance mostly come from a motion invariance condition that involves the motion of who's using the
object. Hence, one can simply think of the previously used object identifier symbols as 
indexes that are only formally represented. 

\section{Dealing with attached objects}
The way we conquer the affordance, stated by Eq.~\ref{AffordanceMO} works for both attached and detached 
objects, since their movement is not necessary. The affordance comes from people who are using 
the object. However, the way people interact with attached and detached objects is definitely very different.  
We experiment an interaction with objects that can be directly  grasped  that is far away from 
big fixed objects. While  hammers can be grasped and moved so as their motion with respect  to the
environment can  be used for conquering their identity, a building can nether be grasped nor moved.
Yet, humans and attached objects can still interact so as they can get the affordance from
human movements. As we look out the window or open the shutters, the corresponding movement transfers
an affordance. Something similar happens as we walk close home.  Even though a chair is clearly
detached, it is typically fixed as we seat down or stand up. Of course, it can itself slightly move, but 
the affordance is basically gained from the person who's using it. 

\marginpar{\small Attached and detached objets involve a different optical flow; identification
is favored for detached objects.} 
 Because of the structure of the optical flow generated during object-human interaction, it's
 quite obvious that the identity of detached objects can better be gained. On the opposite, for both attached 
 and detached objects the affordance can be similarly gained. There's still a difference, since
 in detached objects the optical flow comes from both humans and objects.
 
 %
 % la differenza tra detached and attached objects è nel fatto che A_{p \bowtie o} è diversa: non ci sono 
 % O, P  ma solo V
 %

\section{Actions and sequences}

\section{Linguistic interactions}

==> bk/h.tex <==
In this section we discuss visual tasks and their intriguing connection
with language. This analysis is motivated by the evidence provided in
nature of excellent visual skills that arise regardless of language. 
At the light of the following analysis, one should consider to start 
go beyond the tradition of computer vision of emphasizing classification tasks.
Visual perception drives different functional tasks in animals, so as 
the human intersection with language must properly be analyzed. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   definition of the formalism of video signals
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Let $\T=[t_{0},t_{1}]$ be the {\em temporal domain} and let $\X \subset \bbR^{2}$ be the retina. 
We  consider the video domain $\D:= \T \times \X$ so as 
	\[
		v : \D \rightarrow \bbR^{d}: \ (t,x) \rightarrow [v_{1}(t,x),\ldots,
		v_{d}(t,x)]^{\prime}
	\]
is the video signal on $\D$. In the classic case of RGB coding, we have $d=3$.
Throughout the paper, $v(\D)$ denotes any video, while we use $\V$ to denote
the universal set of videos, where any video belongs to. Likewise, $v(t,\X)$ denotes
the frame at $t$ and  $\I$ denotes the universal set of images with values $v(t,x) \in \bbR^{d}$.
Clearly, we have $v(\D) \in \V$. Now, humans are capable of providing sophisticated linguistic
representations from video $v(\D) \in \V$, which involve both local and global features. 
Clearly, abstract descriptions of a visual scene do require considerable linguistic skills,
which emerge also at local level when specific words can also be attached to any 
pixel of a given visual frame. Basically, humans are capable of providing a linguistic
description of $v(\D)$ that goes well beyond object classification. The amount of 
visual information is typically so huge that for an appropriate cognitive transcription at
linguistic level to take place one cannot rely on classification, but  must necessarily
involve the compositional structure of language. This kind of difficulty clearly emerges
when trying to provide a linguistic description to blind people, a task which is quite
difficult also for humans. 

\section{Pixel-wise and abstract visual interpretations}
\label{PW-ABS-VI-sec}
One of the most challenging issues in vision is human ability to jump easily from
pixel-wise to recognition processes and more abstract visual interpretations that
involve frames as well as portions of a video. 
When focussing attention on a certain pixel in a picture, humans can easily make a list of 
``consistent objects'' that reflects the visual information around that pixel. 
Interestingly, that process takes place by automatically adapting a sort of
``virtual window'' used for the decision. This results in the typical detection of objects
with dimension which is growing as that virtual window gets larger and larger. 
More structured objects detected at a given pixel are clearly described by more categories 
than simple primitive objects, but, for humans, the resulting {\em pixel-wise} process is 
surprisingly well-posed from a pure cognitive point of view. However, such a pixel-wise
process seems to emerge upon request; apparently, humans do not carry out such a 
massive computation over all the retina. In addition, there are abstract visual
skills that are unlikely to be attacked by pixel-wise computation. Humans 
provide visual interpretations that goes beyond the truly visual pattern
(see e.g. Kanizsa's illusions). This happens because of the focus of attention,
which somehow locates the object to be processed. As the focus is on the pixel $f(t)$,
the corresponding object can be given an abstract geometrical interpretation by
its shape expressed in term of its contour. While pixel-based processes are based
on all the visual information of the retina associated with a given pixel, 
shape-based recognition emerges when recognizing objects on the basis
of their contour, once we focus attention of a point of the object.  

%
% actions and object affordance
%
Pixel-wise processes can only lead to the emergence of decisions on objects,
which is fact a static concept. It cannot allow us to draw conclusions on actions, whose
understanding does require to involve portions of video. However, like for objects,
the detection of the ``contour of actions'' yields a very useful abstraction. 
The notion {\em object affordance} has a strict connection with that of action.
We carry out many object recognition processes on the basis of actions in which they 
are involved, so as objects are detected because of their role in the scene. 
In other words, the affordance involves the {\em functional role} of objects, which is
used for the emergence of abstract categories. 


\section{The interwound story of vision and language}
In the previous section, we have discussed pixel-wise versus abstract computational
processes aimed at generating labels to be attached to objects and actions.  
We can think of two different alphabets $\Sigma_{p}$ and $\Sigma_{s}$
which refer to words related to {\em pixel-wise and shape-based recognition processes}, respectively. 
For instance, while terms like {\tt eye}, {\tt mouth}, and {\tt face} are typical elements of 
$\Sigma_{p}$, their geometrical description is based on terms in $\Sigma_{s}$. So we 
say that the {\tt face} has an {\tt oval} shape, where {\tt oval} is a typical elements of $\Sigma_{s}$.
%
% constraints? language?
%

Overall, a visual agent performs cognitive tasks by working on $\Sigma_{a} = \Sigma_{p} \lor \Sigma_{s}$.
It is important to point out that $\Sigma_{a}$ is only the alphabet of {\em primitive terms}, since when
dealing with structured objects and actions, visual agents play with concepts described
by additional terms %qui


\iffalse  % actions and affordance
 Let $\A \subset \D$ be and consider the set $v(\A)$. 
An action is a map
\begin{equation}
	a: \V \rightarrow 
\end{equation}
\fi

%
% the role of focus of attention in the production of the sequence-based description of the environment.
%

Basically, the extraction of semantics from video requires 
linguistic descriptions, even at local level, where one is asked to select words 
from the alphabet $\omega \in \Sigma_{s}$. Here we regard any word $\omega$
as a symbol with attached semantics, like in the case of any natural language.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Visual Language Hierarchy
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
% \L_{0}, \CalK_{s}, \CalK_{t} - temporal semantics
%
The most abstract task that humans are capable to face is that of constructing a function
$\mychi_{0}$ as follows
\begin{eqnarray}
		\mychi_{0}: \V \rightarrow \CalL_{0}: v(\D) \rightarrow \mychi_{0}(v(\D)), 
\end{eqnarray}
where $\CalL_{0} \subset \Sigma_{s}^{\star}$ is a type zero language in Chomsky's hierarchy.
This embraces any linguistic report from visual scenes, like, for instance,  movie review. 
In addition to the ability of extracting
information from visual sources, a remarkable specific problem in the construction of
$\mychi_{0}$ is that of properly handing the temporal flow of the frames and to 
provide a semantic representation of the movie actions. Clearly, a movie review does not
only require the ability of extracting a visual representation, but also to properly
understand the actions so as to produce a corresponding descriptions. While cats and
eagles are commonly regarded as animals with very good visual skills, they cannot
produce movie reports. Basically, the sentence  $\mychi_{0}(v(\D)) \in \Sigma_{s}^{\star}$
is expected to be taken from a language $\CalL_{0}$ of highest level in Chomsky classification,
which is denoted by $\CalL_{0}$. 
%and involves both spatial $\CalK_{s}$ and 
%temporal $\CalK_{t}$ knowledge (see Tab~\ref{LanguageLevTable}). 

Another fundamental visual task is that  of {\em query answer}, that can be regarded as 
\begin{eqnarray}
		\mychi_{0}: \V \times \CalL_{0} \rightarrow \CalL_{0}: v(\D) \rightarrow \mychi_{0}(v(\D)), 
\end{eqnarray}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}
\baselineskip12pt
\vbox{
\mixthree
\hbox{{\bf input} {\becomes} {\bf semantic description}}	&\hfil\rm {\bf Remarks}\cr
\noalign{\hrule\medskip}
\mychi_{0}(v(\D))\becomes \CalL_{0}	&The language involves ordinary human scene descriptions.  Spatial and knowledge levels are both involved. \cr
\mychi_{1}(v(t,\X))\becomes \CalL_{0} &The language involves ordinary human picture descriptions. Spatial  knowledge is only involved.\cr
\mychi_{2}(t,x,v(t,\X))\becomes \CalL_{-1}		& The language consists of a list of words (language degeneration,  no ordering), that is $ \CalL_{-1} \subset \Sigma_{s}^{\star}$ only.\cr.
\mychi_{3}(t,x,v(t,\X))\becomes \CalL_{-2}		& The language consists of a vector of words (language degeneration,  no order). Unlike $\CalL_{-1}$, the number of symbols is known in advance.\cr
\endmix}
\caption{Hierarchical structure of semantic labeling.}
\label{LanguageLevTable}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%
% \L_{0}, \CalK_{s} - no temporal semantics
%
A simplified version and more realistic formulation of semantic labeling, when actions
are not the target, is the one in which 
\begin{eqnarray}
	\mychi_{1}:  \I \rightarrow \CalL_{0}: (v(t,\X)) \rightarrow 
	\mychi_{1}(v(t,\X)).
\end{eqnarray}
This tasks still requires $\CalL_{0}$ for linguistic description, but only spatial knowledge
$\CalK_{s}$ is needed, since, unlike the previous case, there is no temporal processing required. 

%
% \L_{-1}
%
A dramatic drop of complexity arises when asking the agent to provide visual skills 
on $v(t,\X)$ while focussing attention to $(t,x)$. This is described by
\begin{eqnarray}
	\mychi_{2}: \D \times \I \rightarrow \Sigma_{s}: (t,x,v(t,\X)) \rightarrow 
	\mychi_{2}(t,x,v(t,\D)) ,
\end{eqnarray}
Basically, while the decision is based on 
$u(t,x) = (t,x,v(t,\X)) \in \U$,
which represents quite an unusual granule of information with respect to what is typically processed
in machine learning and pattern recognition, this time there is no linguistic description, since
we only expected the agent to return a list of symbols of  $\Sigma_{s}$.
This simplifies dramatically the overall problem, thus contributing to decoupling 
visual and semantic processes. It is worth mentioning that the dramatic reduction of complexity in 
the semantic processes is paired with the emergence of focus of attention, namely with
decisions based on $u(t,x) \in \U$.
In principle, one can expect semantic labeling of $(t,x)$ by means of a single $\omega \in \Sigma_{s}$,
but in some cases  dozens of  words might be associated with $u(t,x)$. 
While the linguistic structure degenerates, we are still in presence of a compositional 
structure, so as the agent might generate remarkable lengthy sentences of pertinent words $\Sigma_{s}^{\star}$. \\

\section{On nowadays collapse of vision to classification}
\label{CollapseClassSec}
%
% \L_{-2}
%
An additional simplification on the semantic level arises when considering that the 
process of generating the words  $\omega \in \Sigma^{\star}$  can be thought of as
a compositional process based on a set $\Sigma_{d}$ of ``dummy symbols", so as
\begin{eqnarray}
	\mychi_{3}: \D \times \I \rightarrow \Sigma_{d}: (t,x,v(t,\X)) \rightarrow 
	\mychi_{3}(t,x,v(t,\D)) ,
\end{eqnarray}
 
Basically, the transition from $\mychi_{2}(\cdot)$ to $\mychi_{3}(\cdot)$ involves
a further definitive linguistic simplification, which restricts the symbolic description 
from $\Sigma_{s}^{\star}$ to $\Sigma_{d}$. In so doing, all the complexity is now
on the visual side, which requires decisions based on $u(t,x)$, so as we are
finally in front of a {\em classification problem}. 
This description of visual tasks makes it clear that in order to conquer 
abstract computer vision skills, any agent does require to address both issues
of input representation and linguistic descriptions. We claim that any 
systematic approach to vision cannot avoid to face the issue of decoupling 
the classification of visual features, with symbols in $\Sigma_{d}$, and the
appropriate linguistic description.  

%
% problems that arises when ignoring the decoupling
%
Let us analyze the problems connected with the construction of $\mychi_{0}$ and
$\mychi_{1}$, which both operate on global input representation, thus disregarding
any focus of attention mechanism. The complexity can be promptly appreciated also
in the simplest task $\mychi_{1}$. Clearly, it cannot be regarded as a classification
%problem\footnote{See \url{http://www.stat.ucla.edu/~sczhu/Comic_pictures}.},
since the agent is expected to provide truly linguistic descriptions. On top of that,
when dealing with unrestricted visual environments, the interpretation of 
$v(t,\X)$ is trapped into the chicken-egg dilemma on whether classification of objects or
segmentation must take place first. This is due to the absence of any focus of attention,
which necessarily leads to holistic mechanisms of information extraction.
Unfortunately, while holistic mechanisms are required at a certain level of abstraction,
the direct process of  $v(t,\X)$ do not offer the right source for their activation.
Basically, there is no decoupling between the visual source and its linguistic description.  

%
% Hierarchical structure
%
Interestingly, this decoupling takes place when separating
$\mychi_{3}(\cdot)$ with respect to the others. 
The development of abstract levels
of description can follow the chaining process
\begin{equation}
	\boxed{\U \stackrel{\mychi_{3}}{\longrightarrow} \Sigma_{d} } 
	\stackrel{\mychi_{2}}{\longrightarrow} \Sigma_{s}^{\star}
	\stackrel{\mychi_{1}}{\longrightarrow} (\Sigma_{s}^{\star},\CalL_{0},\CalK_{s})
	\stackrel{\mychi_{0}}{\longrightarrow} (\Sigma_{s}^{\star},\CalL_{0},\CalK_{s},\CalK_{t}),
\end{equation}
where $\mychi_{3}(\cdot)$ is the only one which deals with the visual signal. All the other
functions involve symbolic processes at different levels of abstraction. 
From one side, $\mychi_{3}(\cdot)$ exploits the focus of attention on $(t,x) \in \D$ to 
better process the visual information, and, from the other side, it gets rid of any linguistic
structure by relying on the classification of dummy symbols. 

\section{Scholia}



==> bk/misc/llncs2e/mydefs.tex <==

% For et al.'ing things
\newcommand{\etal}{{\em et al.\/}}
\def\annote#1{\par {\bf #1}\par}


%\def\NaturalSet{\mbox{I\hspace*{-0.16em}N}}
\def\RealSet{\mbox{I\hspace*{-0.16em}R}}

\def\NaturalSet{\mbox{$I\!\! N$}}
%\def\RealSet{\mbox{$I\!\!R$}}
%\def\func#1{\mbox{$#1(\cdot)$}}

\def\N{\mbox{$I\!\! N$}}
\def\R{\mbox{$I\!\!R$}}
\def\C{\mbox{\rm C}}

\def\QED{\protect{\flushright{$\Box$}}}
%\def\QED{\mbox{\rule[0pt]{1.5ex}{1.5ex}}}
%\def\qed{\hspace*{\fill}~\protect{\QED}}
%\def\ONE{\Huge{\bf 1}\hspace{-.1cm}\normalsize{\mbox {\bf I}}}
%\def\ONE{{\bf 1}\hspace{-.3cm}{\mbox {\bf I}}}
\def\ONES{\mbox{\unboldmath $1$}}
%\def\ONES{\mbox{\unboldmath 1} \hspace{-.1cm}\normalsize{\mbox {\unboldmath I}}}
\def\ZERO{\bf 0}

\def\sequence#1#2#3{#1^{#3\choose #2}}
\def\chain{\oplus}
\def\quantize#1{\ulcorner #1 \lrcorner}
\def\path{\leadsto}
\def\nil{\mbox{\boldmath $0$}} 
\def\ONE{\mbox{\boldmath $1$}} 
\def\BBox{\vrule height 1.2ex width 1.2ex depth -.1ex}
\def\warp{\bowtie}
\def\RealSet{\mbox{$I\!\!R$}}


\def\smap{F}
\def\gmap{\mbox{\Large{$\tau$}}}
\def\tmap{f}


\def\shape#1{\rm }
\def\ot{\overline{t}}
\def\osigma{\overline{\sigma}}
\def\Set{\mbox{$\mbox{\sc set}$}}
\def\Reset{\mbox{$\mbox{\sc reset}$}}
\def\Nil{\mbox{$\mbox{\sc nil}$}}
\def\Not{\mbox{$\mbox{\sc not}$}}
\def\False{\mbox{$\mbox{\sc false}$}}
\def\True{\mbox{$\mbox{\sc true}$}}

\def\Action{$\mbox{\boldmath ${\cal A}$}$}

\def\A{\mathscr{A}}
\def\X{\mathscr{X}}
\def\Y{\mathscr{Y}}
\def\Z{\mathscr{Z}}
\def\M{\mathscr{M}}
\def\O{\mathscr{O}}
\def\T{\mathscr{T}}
\def\U{\mathscr{U}}
\def\V{\mathscr{V}}
\def\S{\mathscr{S}}
\def\F{\mathscr{F}}
\def\D{\mathscr{D}}
\def\I{\mathscr{I}}

\def\pa{\mbox{pa}}
\def\vert{\mbox{vert}}
\def\de{\mbox{de}}
\def\det{\mbox{det}}
\def\dim{\mbox{dim}}
\def\sign{\mbox{sign}}
\def\diag{\mbox{diag}}
\def\ln{\mbox{ln}}
%\def\arg{\mbox{\shape{n}\selectfont arg}}
\def\softmax{\mbox{softmax}}
\def\argmax{\mathop{\operator@font argmax}}
\def\argmin{\mathop{\operator@font argmin}}

\def\BA{\mbox{\boldmath $A$}}
\def\BB{\mbox{\boldmath $B$}}
\def\BC{\mbox{\boldmath $C$}}
\def\BD{\mbox{\boldmath $D$}}
\def\BG{\mbox{\boldmath $G$}}
\def\BF{\mbox{\boldmath $F$}}
\def\BI{\mbox{\boldmath $I$}} 
\def\BPhi{\mbox{\boldmath $\Phi$}}
\def\BR{\mbox{\boldmath $R$}}
\def\BS{\mbox{\boldmath $S$}} 
\def\BL{\mbox{\boldmath $L$}} 
\def\BTheta{\mbox{\boldmath $\Theta$}}
\def\Bsigma{\mbox{\boldmath $\sigma$}}
\def\BU{\mbox{\boldmath $U$}} 
\def\BH{\mbox{\boldmath $H$}} 
\def\BM{\mbox{\boldmath $M$}}
\def\BN{\mbox{\boldmath $N$}}
\def\BP{\mbox{\boldmath $P$}} 
\def\BT{\mbox{\boldmath $T$}}
\def\BV{\mbox{\boldmath $V$}} 
\def\BX{\mbox{\boldmath $X$}}
\def\BB{\mbox{\boldmath $B$}}
\def\BC{\mbox{\boldmath $C$}}
\def\BR{\mbox{\boldmath $R$}}
\def\BY{\mbox{\boldmath $Y$}} 
\def\BW{\mbox{\boldmath $W$}}
\def\BZ{\mbox{\boldmath $Z$}}
\def\B0{\mbox{\boldmath $0$}}
\def\Balpha{\mbox{\boldmath $\alpha$}}
\def\Ba{\mbox{\boldmath $a$}}
\def\Bbeta{\mbox{\boldmath $\beta$}}
\def\Bb{\mbox{\boldmath $b$}}
\def\Bc{\mbox{\boldmath $c$}}
\def\Bd{\mbox{\boldmath $b$}}
\def\Bgamma{\mbox{\boldmath $\gamma$}}
\def\Bdelta{\mbox{\boldmath $\delta$}}
\def\BDelta{\mbox{\boldmath $\Delta$}}
\def\Beta{\mbox{\boldmath $\eta$}}
\def\Be{\mbox{\boldmath $e$}}
\def\Bepsilon{\mbox{\boldmath $\epsilon$}}
\def\Bf{\mbox{\boldmath $f$}}
\def\Blambda{\mbox{\boldmath $\lambda$}}
\def\Bg{\mbox{\boldmath $g$}}
\def\Bmu{\mbox{\boldmath $\mu$}} 
\def\Bnu{\mbox{\boldmath $\nu$}} 
\def\Bm{\mbox{\boldmath $m$}}
\def\Bo{\mbox{\boldmath $o$}}
\def\Bphi{\mbox{\boldmath $\phi$}}
\def\Bpi{\mbox{\boldmath $\pi$}}
\def\Bpsi{\mbox{\boldmath $\psi$}}
\def\Bpi{\mbox{\boldmath $\pi$}}
\def\Bp{\mbox{\boldmath $p$}}
\def\Bq{\mbox{\boldmath $q$}}
\def\Br{\mbox{\boldmath $r$}}
\def\Bs{\mbox{\boldmath $s$}}
\def\Btheta{\mbox{\boldmath $\theta$}}
\def\Bdelta{\mbox{\boldmath $\delta$}}
\def\Bomega{\mbox{\boldmath $\omega$}}
\def\Bu{\mbox{\boldmath $u$}}
\def\Bvarphi{\mbox{\boldmath $\varphi$}}
\def\Bvartheta{\mbox{\boldmath $\vartheta$}}
\def\Bvarsigma{\mbox{\boldmath $\varsigma$}}
\def\Bv{\mbox{\boldmath $v$}}
\def\Bw{\mbox{\boldmath $w$}} 
\def\Bxi{\mbox{\boldmath $\xi$}}
\def\Bx{\mbox{\boldmath $x$}}
\def\Bd{\mbox{\boldmath $d$}}
\def\By{\mbox{\boldmath $y$}} 
\def\Bzeta{\mbox{\boldmath $\zeta$}}
\def\Bz{\mbox{\boldmath $z$}}

\def\EQ{\!=\!}
\def\Given{\mbox{$\: \bigl | \bigr. \:$}}
\def\MAX{\mbox{\sc max}}
\def\MIN{\mbox{\sc min}}
\def\Overq{{\overline{q}}}
\def\Pr{\mbox{P}}
\def\given{\mbox{$\: | \:$}}

\def\vectw#1#2{\!\left[\!\!\begin{array}{r}#1\\#2\end{array}\!\!\right]\!}

\def\ivector#1{\sfmath{I}_{[#1]}}
\def\CalA{{\cal A}}
\def\CalB{{\cal B}}
\def\CalC{{\cal C}}
\def\CalD{{\cal D}}
\def\CalE{{\cal E}}
\def\CalF{{\cal F}}
\def\CalG{{\cal G}}
\def\CalH{{\cal H}}
\def\CalI{{\cal I}}
\def\CalK{{\cal K}}
\def\CalL{{\cal L}}
\def\CalM{{\cal M}}
\def\CalN{{\cal N}}
\def\CalO{{\cal O}}
\def\CalP{{\cal P}}
\def\CalQ{{\cal Q}}
\def\CalR{{\cal R}}
\def\CalS{{\cal S}}
\def\CalT{{\cal T}}
\def\CalU{{\cal U}}
\def\CalV{{\cal V}}
\def\CalW{{\cal W}}
\def\CalX{{\cal X}}
\def\CalY{{\cal Y}}
\def\CalZ{{\cal Z}}
\def\VecCalE{{\cal{\vec{E}}}}
\def\Alphabet{{\cal A}}
\def\Real{\mbox{$\mathbb{R}$}}
\def\AND{\mbox{${\cal B}_\wedge$}}
\def\OR{\mbox{${\cal B}_\vee$}}

\def\istar{\mbox{$\CalI^\star$}}
% \def\EqDef{\doteq}
\def\EqDef{\buildrel \rm def \over =}

\def\RefFig#1{Figure~\ref{#1}}
\def\RefTab#1{Table~\ref{#1}}
\def\RefEq#1{(\ref{#1})}
\def\RefEqs#1#2{(\ref{#1},\ref{#2})}
\def\RefCh#1{Chapter \ref{#1}}
\def\RefSect#1{\S~\ref{#1}}
\def\RefSec#1{\S~\ref{#1}}
\def\RefSub#1{\S~\ref{#1}}
\def\RefDef#1{Definition~\ref{#1}}
\def\RefTh#1{Theorem~\ref{#1}}
\def\RefTh#1{Conjecture~\ref{#1}}
\def\cdw#1{{\em \underline{#1}}}
\def\RealSet{\mbox{$I\! \! R$}}
\newcommand{\bbR}{{\mathbb{R}}}
\newcommand{\bbN}{{\mathbb{N}}}
\newcommand{\bbK}{{\mathbb{K}}} %I've added this line to compile hf2.tex Alessandro.

% An list-like environment that indents second, etc. lines of each item.
\newenvironment{defs}%
{\begin{list}{}{\setlength{\itemindent}{-\leftmargin}\setlength{\itemsep}{0pt}\setlength{\parsep}{0pt}}}%
{\end{list}}

% shrink and rotate everything for a two-pages on 1 printing using dvips.
%\input reduce.tex

% ``\heading'' is like a subsubsubsection, and takes a single argument.
% \newcommand{\heading}[1]{ \medskip
%         {\setlength{\parindent}{0in} \bf #1}
%         \nopagebreak
%         }

% ``\comment'' takes a single argument
\newcommand{\comment}[1]{}


% Local Variables: 
% mode: latex
% TeX-master: "main"
% End: 


==> bk/p_copy.tex <==

\preface\vspace{-4cm}
%
% Posing the right questions
%
A good way to attack important problems is to pose the right question. This mostly 
a book of questions more than of concrete solutions, yet it  can open a debate and solicit answers. 
Posing the right questions does require a big picture in mind and the need to identify 
reasonable intermediate steps. As I began the contamination with computer vision 
a lot questions crossed my mind that I think make this topic really fascinating.
How can animals conquer visual skills without requiring ``intensive supervision''?
What is the role of time? What is the relationship between the time of the agent  and the time of the environment?
Can animals see in a world of shuffled frames?
How can we perform semantic pixel labelling without receiving one specific single supervision?
Why has the brain reached a hierarchical organization and two functionally separated  mainstreams?
Why top level visual skills are achieved in nature thanks to focus of attention? What is driving eye movements?
Why does it take 8-12 months for newborns to achieve adult visual acuity?
How can we develop ``linguistic focusing mechanisms''   that can drive the process of object recognition?

%
% The success of deep supervised learning
%
By and large, the remarkable progress in visual object recognition in the last few years is 
attributed to the availability of huge labelled data paired with strong and suitable computational
resources. This has opened the doors to the massive use of deep learning,
which has led to remarkable improvements on common benchmarks.
While subscribing this view, in this book we claim that the time has come to 
begin working towards a deeper understanding of visual computational processes, that
instead of being regarded as applications of general purpose machine learning algorithms,
are likely to require appropriate learning schemes. The major claim is that while facing 
nowadays object recognition problems we have been working a problem that is
significantly more difficult than the one offered by nature. This is due to learning
algorithms that are working on images while neglecting the crucial role of frame
temporal coherence. It looks like Nature did a nice job by using time to sew all the video frames. When computer scientists began to cultivate the idea of interpreting natural
video, in order to simplify the problem they remove time, the connecting wire between
frames. As a consequence, video turned into huge collections of images, where 
most of temporal coherence was lost. 
At a first glance, this is reasonable, especially if you consider that video were
traditionally heavy data sources. However, a closer look reveals that 
we are in fact neglecting a fundamental clue to interpret visual information, 
and that we end up into problems where the extraction of the visual concepts 
can only be based on  spatial  regularities.
% Throughout the book, we mostly address the limitations of nowadays approaches to 
% computer vision, and discuss how the evolution  of 
%the tradition of image recognition towards visual recognition might give rise to 
%remarkable advances in the field of computer vision.
%This work comes from a book chapter originated by an invited talk at the International
%Workshop on Neural Networks for Pattern Recognition. 
%The circulation of the chapter gave rise to interesting discussions with colleagues, 
%especially after my presentation at the FBK, Trento, within the  ``Edge of AI''  
%contributions. As I decided to enrich the material to compose the book, I was early
%in front of the question on the appropriateness of the title I used for the chapter. 
%It was in fact the source of some ``velate'' criticisms that I couldn't ignore. 
%Interestingly, after having evaluated careful the essence of the message the
%book is supposed to deliver, we decided to stick with the same title and defend 
%our position:
Computer vision is definitely one of the most successful topics
in computer science, especially if we consider its impressive impact in 
real-world applications in the last few years. Yet, it is a formidable collection of
tools and techniques conceived to face specific tasks, while we are still 
missing the big picture! How is that 
tasks as different as automatic navigation and linguistic scene interpretation
is solved by humans with no apparent difficulty? 
While we are still likely missing human reliable spotting of visual clues, we
are frankly far away from our spectacular ``reading'' of visual scenes
by abstract linguistic representations of the world.

This book offers a unified view that is driven by the principle of capturing the underlying 
information-based laws of vision. While we rely on the representational power of 
deep architecture with convolutional structure, we emphasize learning mechanisms that
are strongly based on motion. Instead of addressing the rich literature on invariance
and equivariance we propose the uniform invariance properties that arise when tracking
objects. This opens the doors to understand visual computational processes regardless of 
biology and computer architectures. The focus on motion invariance feature extraction makes it
possible to understand  how can animals of different species 
conquer the visual skills they required during the evolution. Moreover, this also
sets the relationship of vision and language in a truly novel framework from which 
also computer vision that might benefit.\\
~\\
Marco Gori, Siena, May 2021


==> bk/references.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
\biblstarthook{References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} If the citatiion in the text is numbered, the reference list should be arranged in ascending order. If the citation in the text is author/year, the reference list should be \textit{sorted} alphabetically and if there are several works by the same author, the following order should be used:
\begin{enumerate}
\item all works by the author alone, ordered chronologically by year of publication
\item all works by the author with a coauthor, ordered alphabetically by coauthor
\item all works by the author with several coauthors, ordered chronologically by year of publication.
\end{enumerate}
The \textit{styling} of references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}, see \url{http://www.issn.org/en/node/344}} depends on the subject of your book:
\begin{itemize}
\item The \textit{two} recommended styles for references in books on \textit{mathematical, physical, statistical and computer sciences} are depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI} and ~\cite{phys-online, phys-mono, phys-journal, phys-DOI, phys-contrib}.
\item Examples of the most commonly used reference style in books on \textit{Psychology, Social Sciences} are~\cite{psysoc-mono, psysoc-online,psysoc-journal, psysoc-contrib, psysoc-DOI}.
\item Examples for references in books on \textit{Humanities, Linguistics, Philosophy} are~\cite{humlinphil-journal, humlinphil-contrib, humlinphil-mono, humlinphil-online, humlinphil-DOI}.
\item Examples of the basic Springer Nature style used in publications on a wide range of subjects such as \textit{Computer Science, Economics, Engineering, Geosciences, Life Sciences, Medicine, Biomedicine} are ~\cite{basic-contrib, basic-online, basic-journal, basic-DOI, basic-mono}. 
\end{itemize}
}

\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution 
\bibitem{science-contrib} Broy, M.: Software engineering --- from auxiliary to key technologies. In: Broy, M., Dener, E. (eds.) Software Pioneers, pp. 10-13. Springer, Heidelberg (2002)
%
% Online Document
\bibitem{science-online} Dod, J.: Effective substances. In: The Dictionary of Substances and Their Effects. Royal Society of Chemistry (1999) Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{science-mono} Geddes, K.O., Czapor, S.R., Labahn, G.: Algorithms for Computer Algebra. Kluwer, Boston (1992) 
%
% Journal article
\bibitem{science-journal} Hamburger, C.: Quasimonotonicity, regularity and duality for nonlinear systems of partial differential equations. Ann. Mat. Pura. Appl. \textbf{169}, 321--354 (1995)
%
% Journal article by DOI
\bibitem{science-DOI} Slifka, M.K., Whitton, J.L.: Clinical implications of dysregulated cytokine production. J. Mol. Med. (2000) doi: 10.1007/s001090000086 
%
\bigskip

% Use the following (APS) syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Online Document
\bibitem{phys-online} J. Dod, in \textit{The Dictionary of Substances and Their Effects}, Royal Society of Chemistry. (Available via DIALOG, 1999), 
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{phys-mono} H. Ibach, H. L\"uth, \textit{Solid-State Physics}, 2nd edn. (Springer, New York, 1996), pp. 45-56 
%
% Journal article
\bibitem{phys-journal} S. Preuss, A. Demchuk Jr., M. Stuke, Appl. Phys. A \textbf{61}
%
% Journal article by DOI
\bibitem{phys-DOI} M.K. Slifka, J.L. Whitton, J. Mol. Med., doi: 10.1007/s001090000086
%
% Contribution 
\bibitem{phys-contrib} S.E. Smith, in \textit{Neuromuscular Junction}, ed. by E. Zaimis. Handbook of Experimental Pharmacology, vol 42 (Springer, Heidelberg, 1976), p. 593
%
\bigskip
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Psychology, Social Sciences"
%
%
% Monograph
\bibitem{psysoc-mono} Calfee, R.~C., \& Valencia, R.~R. (1991). \textit{APA guide to preparing manuscripts for journal publication.} Washington, DC: American Psychological Association.
%
% Online Document
\bibitem{psysoc-online} Dod, J. (1999). Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/Effective substances.} Cited 15 Jan 1999.
%
% Journal article
\bibitem{psysoc-journal} Harris, M., Karper, E., Stacks, G., Hoffman, D., DeNiro, R., Cruz, P., et al. (2001). Writing labs and the Hollywood connection. \textit{J Film} Writing, 44(3), 213--245.
%
% Contribution 
\bibitem{psysoc-contrib} O'Neil, J.~M., \& Egan, J. (1992). Men's and women's gender role journeys: Metaphor for healing, transition, and transformation. In B.~R. Wainrig (Ed.), \textit{Gender issues across the life cycle} (pp. 107--123). New York: Springer.
%
% Journal article by DOI
\bibitem{psysoc-DOI}Kreger, M., Brindis, C.D., Manuel, D.M., Sassoubre, L. (2007). Lessons learned in systems change initiatives: benchmarks and indicators. \textit{American Journal of Community Psychology}, doi: 10.1007/s10464-007-9108-14.
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Humanities, Linguistics, Philosophy"
%
\bigskip
%
% Journal article
\bibitem{humlinphil-journal} Alber John, Daniel C. O'Connell, and Sabine Kowal. 2002. Personal perspective in TV interviews. \textit{Pragmatics} 12:257--271
%
% Contribution 
\bibitem{humlinphil-contrib} Cameron, Deborah. 1997. Theoretical debates in feminist linguistics: Questions of sex and gender. In \textit{Gender and discourse}, ed. Ruth Wodak, 99--119. London: Sage Publications.
%
% Monograph
\bibitem{humlinphil-mono} Cameron, Deborah. 1985. \textit{Feminism and linguistic theory.} New York: St. Martin's Press.
%
% Online Document
\bibitem{humlinphil-online} Dod, Jake. 1999. Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999
%
% Journal article by DOI
\bibitem{humlinphil-DOI} Suleiman, Camelia, Daniel C. O'Connell, and Sabine Kowal. 2002. `If you and I, if we, in this later day, lose that sacred fire...': Perspective in political interviews. \textit{Journal of Psycholinguistic Research}. doi: 10.1023/A:1015592129296.
%
%
%
\bigskip
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Computer Science, Economics, Engineering, Geosciences, Life Sciences"
%
%
% Contribution 
\bibitem{basic-contrib} Brown B, Aaron M (2001) The politics of nature. In: Smith J (ed) The rise of modern genomics, 3rd edn. Wiley, New York 
%
% Online Document
\bibitem{basic-online} Dod J (1999) Effective Substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Journal article by DOI
\bibitem{basic-DOI} Slifka MK, Whitton JL (2000) Clinical implications of dysregulated cytokine production. J Mol Med, doi: 10.1007/s001090000086
%
% Journal article
\bibitem{basic-journal} Smith J, Jones M Jr, Houghton L et al (1999) Future of health insurance. N Engl J Med 965:325--329
%
% Monograph
\bibitem{basic-mono} South J, Blass B (2001) The future of modern genomics. Blackwell, London 
%
\end{thebibliography}

